SOK-Bench: A Situated Video Reasoning Benchmark with Aligned Open-World Knowledge

Learning commonsense reasoning from visual contexts and scenes in real-world is a crucial step toward advanced artificial intelligence. However, existing video reasoning benchmarks are still inadequate since they were mainly designed for factual or situated reasoning and rarely involve broader knowledge in the real world. Our work aims to delve deeper into reasoning evaluations, specifically within dynamic, open-world, and structured context knowledge. We propose a new benchmark (SOK-Bench), consisting of 44K questions and 10K situations with instance-level annotations depicted in the videos. The reasoning process is required to understand and apply situated knowledge and general knowledge for problem-solving. To create such a dataset, we propose an automatic and scalable generation method to generate question-answer pairs, knowledge graphs, and rationales by instructing the combinations of LLMs and MLLMs. Concretely, we first extract observable situated entities, relations, and processes from videos for situated knowledge and then extend to open-world knowledge beyond the visible content. The task generation is facilitated through multiple dialogues as iterations and subsequently corrected and refined by our designed self-promptings and demonstrations. With a corpus of both explicit situated facts and implicit commonsense, we generate associated question-answer pairs and reasoning processes, finally followed by manual reviews for quality assurance. We evaluated recent mainstream large vision-language models on the benchmark and found several insightful conclusions. For more information, please refer to our benchmark at www.bobbywu.com/SOKBench.

==> algorithms/alg1.tex <==
\begin{algorithm}[th]
\small
\SetKwFunction{FLLM}{LLM}
\SetKwFunction{FVL}{VL}
\SetKwFunction{FSituatedKnowledgeGraph}{GetSKG}

\KwInput{video $v$, manual annotations of events $\{y_{t}\}$, Large Language Model \FLLM, Vision-Language Model \FVL, generation goal instructions $\{ \omega \}$, output format instructions $\{ \phi \}$}

\Fn{\FSituatedKnowledgeGraph{$v$, $\{y_{t}\}$}}{
    % \Repeat{} {
    % }
    \KwInit{Situated Knowledge Graph $\mbox{\boldmath$G$}_{v} = [ \ ]$}
    
    \tcc{1 parse objs and acts from annotations and output in JSON format}
    \textbf{objs} $\{o_{i}\} \leftarrow$ \FLLM{$\langle \{y_{t}\}\ |\ \omega_{obj}, \phi_{obj} \rangle$} \;
    \textbf{acts} $\{a_{t}\} \leftarrow$ \FLLM{$\langle \{y_{t}\}\ |\ \omega_{act}, \phi_{act} \rangle$} \;
    
    \tcc{2 obtain obj attributes and obj-obj relationships}
    sample \textbf{frames} with timestamps $\{f_{t^{*}}\} \leftarrow v$\;
    \For{each $f_{t^{*}} \in \{f_{t^{*}}\}$}{
        extract \textbf{obj} strings from frames \\ $o^{*} \leftarrow$ \FVL{$\langle f_{t^{*}}\ |\ \omega_{obj}^{*} \rangle$} \;
        parse \textbf{objs} in JSON format \\ $\{o_{i}^{*}\} \leftarrow$ \FLLM{$\langle o^{*}\ |\ \phi_{obj}^{*} \rangle$} \;
        \tcp{check missing objs (\FVL may fail to recognize objs in frames)}
        \For{each $o_{i} \in \{o_{i}\}$}{
            \If{$o_{i}$ in $t^{*}$ \& $o_{i} \notin \{o_{i}^{*}\}$}{
                $\{o_{i}^{*}\} := \{o_{i}^{*}\} + o_{i}$
            }
        }
        \tcp{obj attributes}
        \For{each $o_{i}^{*} \in \{o_{i}^{*}\}$}{
            get \textbf{obj attributes} \\ $attr_{i} \leftarrow$ \FVL{$\langle f_{t^{*}}\ |\ \omega_{attr}^{i} \rangle$} \;
            \tcp{add edges of <time, obj> and <obj, attribute> to SKG}
            add edge $(t^{*}, o_{i}^{*})$ to $\mbox{\boldmath$G$}_{v}$ \;
            add edge $(o_{i}^{*}, attr_{i})$ to $\mbox{\boldmath$G$}_{v}$ \;
            % \tcp{add the edge of <timestamp, obj, attribute> to VG}
        }
        \tcp{obj-obj spatial relations}
        \For{each pair $(o_{i}^{*}, o_{j}^{*})$}{
            get \textbf{obj-obj spatial relations} \\ $re_{i, j} \leftarrow$ \FVL{$\langle f_{t^{*}}, \omega_{re}^{i,j} \rangle$} \;
            \tcp{add edge of <obj i, relationship, obj j> to SKG}
            add edge $(o_{i}^{*}, re_{i,j}, o_{j}^{*})$ to $\mbox{\boldmath$G$}_{v}$ \;
        }
    }

    \tcc{3 align acts with objs}
    \For{each $f_{t^{*}} \in \{f_{t^{*}}\}$, each $a_{t} \in \{a_{t}\}$}{
        \For{each $o_{i}^{*} \in \{o_{i}^{*}\}$} {
            \If{ $t^{*}$ in $t$ \& $o_{i}^{*}$ in $a_{t}$ } {
                \tcp{add edges of <act, obj> to SKG}        
                add edge $(a_{t}, o_{i}^{*})$ to $\mbox{\boldmath$G$}_{v}$\;
            }
        }
        \tcp{add edges of <time, act> to SKG} 
        add edge $(t, a_{t})$ to $\mbox{\boldmath$G$}_{v}$\;
    }
    \KwRet $\mbox{\boldmath$G$}_{v}$ \;
}

% \Fn{\FSituatedKnowledgeGraph{}}{
%     % \Repeat{} {
%     % }
%     \For{}{
%         \;
%     }
%     \KwRet $\mbox{\boldmath$G$}_{sk}$ \;
% }

\caption{Situated Knowledge Graph}
\label{algo:situated_knowledge_graph_generation}
\end{algorithm}






% \begin{algorithm}[th]
% \small
% \SetKwFunction{FLLM}{LLM}
% \SetKwFunction{FVL}{VL}
% \SetKwFunction{FSituatedKnowledgeGraph}{GetSituatedKnowledgeGraph}

% \KwInput{video $v$, manual annotations $\{y_{t}\}$, language model \FLLM, vision-language model \FVL, generation goal instructions $\{ \omega \}$, output format instructions $\{ \phi \}$}

% \Fn{\FSituatedKnowledgeGraph{$v$, $\{y_{t}\}$}}{
%     % \Repeat{} {
%     % }
%     \KwInit{Situated Knowledge Graph $\mbox{\boldmath$G$}_{v} = [ \ ]$}
    
%     \tcc{1 parse objs and acts from annotations}
%     \textbf{objs} $\{o_{i}\} \leftarrow$ f_{\FLLM}( y_{t}| \omega_{obj}, \phi_{obj}) \;
    
%     \textbf{acts} $\{a_{t}\} \leftarrow$ g_{\FLLM}( y_{t}| \omega_{act}, \phi_{act}) \;
    
%     \tcc{2 obtain obj attributes and obj-obj relationships}
%     sample \textbf{frames} with timestamps $\{f_{t^{*}}\} \leftarrow v$\;
%     \For{each $f_{t^{*}} \in \{f_{t^{*}}\}$}{
%         \textbf{objs} w/o format $o^{*} \leftarrow$ f_{\FVL}( f_{t^{*}}, \omega_{obj}^{*} ) \;
%         \textbf{objs} w/ format $\{o_{i}^{*}\} \leftarrow$ g_{\FLLM}( o^{*}, \phi_{obj}^{*} ) \;
%         \tcp{check missing objs}
%         \For{each $o_{i} \in \{o_{i}\}$}{
%             \If{$o_{i}$ in $t^{*}$ \& $o_{i} \notin \{o_{i}^{*}\}$}{
%                 $\{o_{i}^{*}\} := \{o_{i}^{*}\} + o_{i}$
%             }
%         }
%         \tcp{obj attributes}
%         \For{each $o_{i}^{*} \in \{o_{i}^{*}\}$}{
%             \textbf{obj attr} $attr_{i} \leftarrow$ \FVL{$\langle f_{t^{*}}, \omega_{attr}^{i} \rangle$} \;
%             % \tcp{add edges of <timestamp, obj> and <obj, attribute>}
%             add edge $(t^{*}, o_{i}^{*})$ to $\mbox{\boldmath$G$}_{v}$ \;
%             add edge $(o_{i}^{*}, attr_{i})$ to $\mbox{\boldmath$G$}_{v}$ \;
%             % \tcp{add the edge of <timestamp, obj, attribute> to VG}
%         }
%         \tcp{obj-obj relationships}
%         \For{each pair $(o_{i}^{*}, o_{j}^{*})$}{
%             \textbf{obj rela} $re_{i, j} \leftarrow$ \FVL{$\langle f_{t^{*}}, \omega_{re}^{i,j} \rangle$} \;
%             % \tcp{add edge of <obj i, relationship, obj j>}
%             add edge $(o_{i}^{*}, re_{i,j}, o_{j}^{*})$ to $\mbox{\boldmath$G$}_{v}$ \;
%         }
%     }

%     \tcc{3 merge acts with objs}
%     \For{each $f_{t^{*}} \in \{f_{t^{*}}\}$, each $a_{t} \in \{a_{t}\}$}{
%         \For{each $o_{i}^{*} \in \{o_{i}^{*}\}$} {
%             \If{ $t^{*}$ in $t$ \& $o_{i}^{*}$ in $a_{t}$ } {
%                 % \tcp{add edges of <timestamp, act> and <act, obj>}        
%                 add edge $(a_{t}, o_{i}^{*})$ to $\mbox{\boldmath$G$}_{v}$\;
%             }
%         }
%         add edge $(t, a_{t})$ to $\mbox{\boldmath$G$}_{v}$\;
%     }
%     \KwRet $\mbox{\boldmath$G$}_{v}$ \;
% }

% % \Fn{\FSituatedKnowledgeGraph{}}{
% %     % \Repeat{} {
% %     % }
% %     \For{}{
% %         \;
% %     }
% %     \KwRet $\mbox{\boldmath$G$}_{sk}$ \;
% % }

% \caption{Situated Knowledge Graph}
% \label{algo:situated_knowledge_graph_generation}
% \end{algorithm}




==> algorithms/alg2.tex <==
\begin{algorithm}[t]
\small
\SetKwFunction{FLLM}{LLM}
\SetKwFunction{FGeneralKnowledgeGraph}{GetGKG}

\KwInput{Situated Knowledge Graph $\mbox{\boldmath$G$}_{v}$, Large Language Model \FLLM, general knowledge aspects $\{\eta_{i}^{obj}\}$, $\{\eta_{i}^{act}\}$ with corresponding knowledge examples $\{\pi_{i}^{obj}\}$, $\{\pi_{i}^{act}\}$, generation goal instructions $\{ \omega \}$, output format instructions $\{ \phi \}$} 
% \KwInit{
% Video Content Graph $\mbox{\boldmath$G$}_{v} = [ \ ]$, \\
% General Knowledge Graph $\mbox{\boldmath$G$}_{gk} = [ \ ]$, \\
% Situated Knowledge Graph $\mbox{\boldmath$G$}_{sk} = [ \ ]$}

% \Fn{\FGeneralKnowledgeGraph{$\mbox{\boldmath$G$}_{v}$, $\{\eta_{i}^{obj}\}$, $\{\eta_{i}^{act}\}$, $\{\pi_{i}^{obj}\}$, $\{\pi_{i}^{act}\}$}}{
\Fn{\FGeneralKnowledgeGraph{$\mbox{\boldmath$G$}_{v}$}}{
    % \Repeat{} {
    % }
    \KwInit{General Knowledge Graph $\mbox{\boldmath$G$}_{gk} = [ \ ]$}
    extract \textbf{objs} $\{o_{i}\}$, \textbf{acts} $\{a_{t}\}$ from $\mbox{\boldmath$G$}_{v}$ \;
    \tcc{1 general knowledge of objs}
    \For{$o_{i} \in \{o_{i}\}$} {
        \tcp{e.g., knowledge aspects of physical, chemical, usage, ...}
        \For{$\eta_{j}^{obj} \in \{\eta_{j}^{obj}\}$, $\pi_{j}^{obj} \in \{\pi_{j}^{obj}\}$}{
            construct generation goal based on one aspect \\ $\omega_{obj}^{*} \leftarrow \langle o_{i}\ |\ \omega_{obj}, \eta_{j}^{obj} \rangle$ \;
            generate \textbf{knowledge} in desired JSON format \\ $\kappa_{i}^{j} \leftarrow$ \FLLM{$\langle \pi_{j}^{obj}, \omega_{obj}^{*}, \phi_{obj} \rangle$} \;
            add edge $( o_{i}, \eta_{j}^{obj}, \kappa_{i}^{j} )$ to $\mbox{\boldmath$G$}_{gk}$\;
        }
    }
    \tcc{2 general knowledge of acts}
    \For{$a_{t} \in \{a_{t}\}$} {
        % \tcp{e.g., general purpose, ways of}
        \For{$\eta_{j}^{act} \in \{\eta_{j}^{act}\}$, $\pi_{j}^{act} \in \{\pi_{j}^{act}\}$}{
            construct generation goal based on one aspect \\ $\omega_{act}^{*} \leftarrow \langle a_{t}\ |\ \omega_{act}, \eta_{j}^{act} \rangle$ \;
            generate \textbf{knowledge} in desired JSON format \\ $\kappa_{i}^{j} \leftarrow$ \FLLM{$\langle \pi_{j}^{act}, \omega_{act}^{*}, \phi_{act} \rangle$} \;
            add edge $( a_{t}, \eta_{j}^{act}, \kappa_{i}^{j} )$ to $\mbox{\boldmath$G$}_{gk}$\;
        }
    }
    \KwRet $\mbox{\boldmath$G$}_{gk}$ \;
}

\caption{General Knowledge Graph}
\label{algo:general_knowledge_graph_generation}
\end{algorithm}

==> algorithms/alg3.tex <==
\begin{algorithm}[t]
\small
\SetKwFunction{FLLM}{LLM}
\SetKwFunction{FSituatedCommonsenseKnowledgeGraph}{GetSCKG}

\KwInput{Situated Knowledge Graph $\mbox{\boldmath$G$}_{v}$, General Knowledge Graph $\mbox{\boldmath$G$}_{gk}$, Large Language Model \FLLM, situated commonsen knowledge aspects $\{\eta_{i}^{obj}\}$, $\{\eta_{i}^{act}\}$, generation goal instructions $\{ \omega \}$, output format instructions $\{ \phi \}$}

\Fn{\FSituatedCommonsenseKnowledgeGraph{$\mbox{\boldmath$G$}_{v}$, $\mbox{\boldmath$G$}_{gk}$}}{
    % \Repeat{} {
    % }
    \KwInit{Situated Commonsense Knowledge Graph $\mbox{\boldmath$G$}_{sk} = [ \ ], J = 2$}
    extract \textbf{objs} $\{o_{i}\}$, \textbf{acts} $\{a_{t}\}$ from $\mbox{\boldmath$G$}_{v}$ \;
    $g_{v} \leftarrow$ texturalized $\mbox{\boldmath$G$}_{v}$ \; 
    \tcc{1 sc knowledge of objs}
    \For{each $\eta_{j}^{obj} \in \{\eta_{j}^{obj}\}$}{
        \tcp{e.g., knowledge aspects of counterfactual and obj contribution}
        situated commonsense examples $\pi_{j} = [ \ ]$ \;
        \Repeat{Finishing J iterations} {
            \For{$o_{i} \in \{o_{i}\}$} {
                $k_{g} \leftarrow$ knowledge related to $o_{i}$ in $\mbox{\boldmath$G$}_{gk}$\;
                $\omega_{obj}^{*} \leftarrow \langle o_{i}\ |\ \omega_{obj}, \eta_{j}^{obj} \rangle$ \;
                $\kappa_{i}^{j} \leftarrow$ \FLLM{$\langle g_{v}, k_{g}, \pi_{j}, \omega_{obj}^{*}, \phi_{obj} \rangle$} \;
                add or update $\kappa_{i}^{j}$ in $\pi_{j}$ \;
                add or update $(o_{i}, \eta_{j}^{obj}, \kappa_{i}^{j})$ in $\mbox{\boldmath$G$}_{sk}$ \;
            }
        }
    }
    \tcc{2 sc knowledge of acts}
    \For{$\eta_{j}^{act} \in \{\eta_{j}^{act}\}$}{
        \tcp{e.g., knowledge aspects of counterfactual and act purpose}
        situated commonsense examples $\pi_{j} = [ \ ]$ \;
        \Repeat{Finishing J iterations} {
            \For{$a_{t} \in \{a_{t}\}$} {
                $k_{g} \leftarrow$ knowledge related to $a_{t}$ in $\mbox{\boldmath$G$}_{gk}$\;
                $\omega_{act}^{*} \leftarrow \langle a_{t}\ |\ \omega_{act}, \eta_{j}^{act} \rangle$ \;
                $\kappa_{i}^{j} \leftarrow$ \FLLM{$\langle g_{v}, k_{g}, \pi_{j}, \omega_{act}^{*}, \phi_{act} \rangle$} \;
                add or update $\kappa_{i}^{j}$ in $\pi_{j}$ \;
                add or update $(a_{t}, \eta_{j}^{act}, \kappa_{i}^{j})$ in $\mbox{\boldmath$G$}_{sk}$ \;
            }
        }
    }
    \KwRet $\mbox{\boldmath$G$}_{sk}$ \;
}

\caption{Situated Commonsense Knowledge Graph}
\label{algo:situated_commonsense_knowledge_graph_generation}
\end{algorithm}

==> sec/materials.tex <==
\subsection{Situated Knowledge Graph (SKG)}
% \subsection{Video Content Graph (VG)}
\label{sec:method_situated_knowledge_graph}

% \input{algorithms/alg1} \bo{Move to supplementary}

% Original Version:
% Video Content Graph $\mbox{\boldmath$G$}_{v}$ describes what we can directly see in the video: objects, object attributes, object spatial relationships, actions, and action temporal relationships. There are three steps to construct the graph.

% It is important to note that we only use vision-language models to process objects, while relying on human annotations for actions, since current video-language models cannot accurately decipher action sequences from videos.

% We add edges representing \textit{(timestamp, object)}, \textit{(object, attribute)}, and \textit{(object$_{i}$, relation, object$_{j}$)} to $\mbox{\boldmath$G$}_{v}$. 
% \noindent\textbf{Merging Actions with Objects.} Finally, we compare the timestamps of frames ${f_{t^{*}}}$ and actions $\{a_{t}\}$ (see Algorithm~\ref{algo:video_content_graph_generation}). If timestamp $t^{*}$ aligns with $t$ and the object $o_{i}^{*}$ from $f_{t^{*}}$ appears in $a_{t}$, we add the corresponding edge which represents \textit{(action, object)} to $\mbox{\boldmath$G$}_{v}$. Also, for each $a_{t}$, we add the edge representing \textit{(timestamp, action)} to show the sequence of actions.

% \bo{rephrased}

Situated knowledge not only represents what is there but also describes the facts, effects, or dynamic processes of activities or events. We construct dynamic situations from videos, and they offer multi-frame event temporality, causality, and dynamics~\cite{buch2022}. 
Recently, more works have presented objects and relations by graphs in real-world dynamic situations~\cite{wu2021star,grunde2021agqa,urooj2023learning} and visual scenes~\cite{ji2020action,zellers2019recognition,hudson2019gqa}. 
We propose Situated Knowledge Graph $\mbox{\boldmath$G$}_{v}$ which extends visual graphs with more visible components in videos. 
The benchmark defines the following fundamental visual entities and relations from dynamic situations of videos: people/objects, attributes, relationships, or actions. 

% \textbf{Objects and Actions.}
We start from the object or action entity generation where they were labeled in the video descriptions from the source video dataset
% and associated with their appeared timestamps 
(\eg, shown in Figure~\ref{fig:graph_gen_pipeline}). 
The descriptions split the dynamic situations by diverse activity moments, and $\{o_{i}\}$ and actions $\{a_{t}\}$ are associated with specific timestamps $\{y_{t}\}$.
Since the original descriptions are human-written text and typically without predefined formats, we utilize the LLMs to parse objects and actions from the description text into lists of them with appeared timestamps. 
We employ a proposed \textit{format} $\phi$$\rangle$ to output ideal formats: key-value lists.
% (\eg, $\langle$[object: tofu, water, cornstarch, ...]$\rangle$ and $\langle$\{``action: ``cut tofu'', ``goal'': ``into square pieces''\}, ...$\rangle$). 
% \bo{check if it's correct or not for the action list}
Notably, some objects are observable in video frames but they were not annotated in the human text annotations. For those objects, we use BLIP2~\cite{li2023blip} to identify objects $\{o_{i}^{*}\}$ in each frame $f_{t^{*}}$ and add them to the initial object list $\{o_{i}\}$.

Situated knowledge not only represents what is there but also describes the facts, effects, or dynamic processes of activities or events. Different from most vision-language benchmarks for commonsense reasoning~\cite{}, we construct dynamic situations from videos, and they offer multi-frame event temporality, causality, and dynamics~\cite{buch2022}. 
Recently, more works have presented objects and relations by graphs in visual situations [XX, XX] and scenes [XX]. 
We propose Situated Knowledge Graph $\mbox{\boldmath$G$}_{v}$ which extends visual graphs with more visible components in videos. 
The benchmark defines the following fundamental visual entities and relations from dynamic situations of videos: \textbf{people/objects}, \textbf{attributes}, \textbf{relationships}, or \textbf{actions}. 

\textbf{Objects and Actions.}
We start from the object or action entity generation where they were labeled in the human-written descriptions from the source video dataset and associated with their appeared timestamps (\eg, shown in Figure~\ref{fig:graph_gen_pipeline}). The descriptions split the dynamic situations by diverse activity moments, and $\{o_{i}\}$ and actions $\{a_{t}\}$ are associated with specific timestamps $\{y_{t}\}$.
Since the original descriptions are human-written text and typically without predefined formats, we utilize the Large Language Model (LLM) to parse objects and actions from the description text into lists of them with appeared timestamps. 
We also employ a proposed \textit{goal} prompt $\omega$ to output the results in a unified \textit{format} $\phi$$\rangle$. 
% \bo{how to use the goal prompt, is the same goal as the goal in the next sentence?}
The \textit{format} shows the ideal output key-value lists (\eg, $\langle$[object: tofu, water, cornstarch, ...]$\rangle$ and $\langle$\{``action: ``cut tofu'', ``goal'': ``into square pieces''\}, ...$\rangle$). 
% \bo{check if it's correct or not for the action list}
Notably, some objects are observable in video frames but they were not annotated in the human text annotations. For those objects, we use BLIP2~\cite{} to identify objects $\{o_{i}^{*}\}$ in each frame $f_{t^{*}}$ and add them to the initial object list $\{o_{i}\}$.

\textbf{Attributes and Relationships.}
Then, we derive object attributes and object-object spatial relationships from sampled keyframes $\{f_{t^{*}}\}$ of video $v$. As depicted in 
Algorithm~\ref{algo:video_content_graph_generation}
, we request MiniGPT4~\cite{openai2023gpt} to response object attributes and object-object spatial relationships with a conversational process. \bo{need to highlight based on the details}
Through the prompts, the method generates various object attributes for visual, physical, and chemical properties and XX relationships (\eg, $\langle$\#Prompt\#: Please describe the tofu in the image in terms of size, shape, color, and texture in one short sentence within 10 words. \#Model\#: The tofus are small, white, sliced squares.$\rangle$). \bo{highlight the attribute selection reason for the given videos with an example; missing the relationship categories}

% \newpage
\begin{figure*}[h]
  %\setlength{\abovecaptionskip}{0pt}
  %\setlength{\belowcaptionskip}{0pt}
  \centering
  \includegraphics[width=18cm]{figures/fig_qa_examples.pdf}
  \caption{Examples of generated question-answer pairs of the benchmark. We demonstrate associated graphs to the QA pairs.}
\label{fig:qa_examples}
\end{figure*}


\section{Situated Commonsense Reasoning Benchmark}
\label{sec:benchmark}


\subsection{Benchmark Overview}
Our benchmark consists of 44K situated commonsense reasoning questions with answers, candidate choices, and 10K trimmed video clips. Each QA pair corresponds to a hypergraph, as illustrated in Figure~\ref{fig:teaser}. These hypergraphs are sampled from a larger Situated Knowledge Graph (see Section~\ref{}), General Knowledge Graph (see Section~\ref{}), and Situated Commonsense Knowledge Graph (see Section~\ref{}). The alignment of hypergraphs with question-answer pairs effectively demonstrates the structured abstraction of video situations and situated knowledge. In addition to the hypergraphs, we provide a rationale that illustrates the reasoning steps taken from the question to the answer (see Figure~\ref{fig:teaser}).

There are 12 types of questions shown in Figure~\ref{fig:dataset_stat}. Notably, the ``Spatiotemporal (ST)'' includes ``obj attributes'', ``obj-obj relations'', ``obj attribute + obj-obj relation'', and ``before/after action'' (see details in Section~\ref{}). `General knowledge (GK)'' covers aspects such as ``physical'', ``chemical'', ``cultural'', and ``usage''. Each question offers four candidate choices, with one annotated as the correct option. As seen in Figure~\ref{fig:dataset_stat}, the distribution of these choices is debiased. Additionally, we utilize LLM to detect and correct any grammatical errors in the questions.

For each question, we provide two answer formats: a direct answer and a multiple-choice format with four options. One option is annotated as the correct choice, while the other three incorrect options are randomly selected from the same knowledge aspect, but related to different objects or actions. Furthermore, we associate each question-answer pair with a corresponding video clip from the raw video, based on the objects and actions mentioned in the text.

\begin{figure}[t]
  %\setlength{\abovecaptionskip}{0pt}
  %\setlength{\belowcaptionskip}{0pt}
  \centering
  \includegraphics[width=8.5cm]{figures/fig_dataset_stat.pdf}
  \caption{\textbf{(a)} Sankey diagram of the 12 question types. \textbf{(b)} Answer distribution among options for each question type. Meaning of abbreviations: O: Object; A: Action; CT: Counterfactual; CB: Contribution; PU: Purpose; R: Reasoning; PO: Possibility; ST: Spatiotemporal; GK: General knowledge.}
\label{fig:dataset_stat}
\end{figure}


\subsection{Benchmark Generation}
We introduce a novel method to efficiently create the benchmark in a controllable and structured manner. If a person were to manually create this benchmark, it would involve four implicit stages: 1) parsing the content of situations, \ie, what can be directly observed in the video; 2) listing related commonsense knowledge as comprehensively as possible; 3) applying reasoning abilities to align situation content components with commonsense knowledge, thereby uncovering hidden logical connections and potential consequences; 4) composing questions and providing answers by synthesizing the aforementioned information.

To enhance the efficiency and structure of this process, we replace human annotators with a Large Language Model (LLM) (\eg, ChatGPT~\cite{}). We design a series of prompt templates that instruct LLM to generate three essential components corresponding to the first three stages: 1) Situated Knowledge Graph (SKG, see Section~\ref{sec:method_situated_knowledge_graph}); 2) General Knowledge Graph (GKG, see Section~\ref{sec:method_general_knowledge_graph}); and 3) Situated Commonsense Knowledge Graph (SKG, see Section~\ref{sec:method_situated_commonsense_knowledge_graph}).

In correspondence with the final stage, we can leverage these graphs to either manually construct question templates (Section~\ref{sec:method_rule_based_qa_gen}) or instruct the LLM (Section~\ref{sec:method_top_down_qa_gen}) to generate question-answer pairs (QAs). This approach enables a clear alignment between the generated QAs and the graphs and corresponding rationale indicating reasoning steps from Q to A. Further details on our generation method are presented in the following sections.

% Lastly, We evaluate the quality of the graphs and QAs through manual assessment.

% Suppose a person manually creates this benchmark, there would be three stages: 1) the person first parses situation content (\ie, what the person can directly see in the video). 2) Next, the person list related commonsense knowledge as much as possible. 3) Finally, the person uses his or her reasoning ability to align the situation content components with commonsense knowledge to reveal hidden logic (\eg, the consequences if an action did not take place). In our study, to make the whole process more effective and in a more structured way, we replace the person with LLM. Corresponding, we design a series of prompt templates to instruct LLM to generate 1) Video Content Graph (VG, see Section~\ref{}), 2) General Knowledgeable Graph (GKG, see Section~\ref{}), and 3) Situated Knowledge Graph (SKG, see Section~\ref{}). Based on the graphs, we may manually build question templates (Section~\ref{}) or instruct LLM (Section~\ref{}) to generate question-answer pairs (QAs). We can present a clear alignment between generated QAs and graphs. Finally, we assess the quality of the graphs and QAs manually.


\subsection{Situated Knowledge Graph (SKG)}
% \subsection{Video Content Graph (VG)}
\label{sec:method_situated_knowledge_graph}

% \input{algorithms/alg1} \bo{Move to supplementary}

% \bo{Original Version:}
% Video Content Graph $\mbox{\boldmath$G$}_{v}$ describes what we can directly see in the video: objects, object attributes, object spatial relationships, actions, and action temporal relationships. There are three steps to construct the graph.

% \bo{need to be clear? move to the end of the first paragraph}
% It is important to note that we only use vision-language models to process objects, while relying on human annotations for actions, since current video-language models cannot accurately decipher action sequences from videos.

% \bo{Original Version:}
% \bo{Describe the graph construction based on the elements}
% We add edges representing \textit{(timestamp, object)}, \textit{(object, attribute)}, and \textit{(object$_{i}$, relation, object$_{j}$)} to $\mbox{\boldmath$G$}_{v}$. 
% \noindent\textbf{Merging Actions with Objects.} Finally, we compare the timestamps of frames ${f_{t^{*}}}$ and actions $\{a_{t}\}$ (see Algorithm~\ref{algo:video_content_graph_generation}). If timestamp $t^{*}$ aligns with $t$ and the object $o_{i}^{*}$ from $f_{t^{*}}$ appears in $a_{t}$, we add the corresponding edge which represents \textit{(action, object)} to $\mbox{\boldmath$G$}_{v}$. Also, for each $a_{t}$, we add the edge representing \textit{(timestamp, action)} to show the sequence of actions.

% \bo{rephrased}

Situated knowledge not only represents what is there but also describes the facts, effects, or dynamic processes of activities or events. We construct dynamic situations from videos, and they offer multi-frame event temporality, causality, and dynamics~\cite{buch2022}. 
Recently, more works have presented objects and relations by graphs in real-world dynamic situations~\cite{wu2021star,grunde2021agqa,urooj2023learning} and visual scenes~\cite{ji2020action,zellers2019recognition,hudson2019gqa}. 
We propose Situated Knowledge Graph $\mbox{\boldmath$G$}_{v}$ which extends visual graphs with more visible components in videos. 
The benchmark defines the following fundamental visual entities and relations from dynamic situations of videos: \textbf{people/objects}, \textbf{attributes}, \textbf{relationships}, or \textbf{actions}. 

\textbf{Objects and Actions.}
We start from the object or action entity generation where they were labeled in the human-written descriptions from the source video dataset and associated with their appeared timestamps (\eg, shown in Figure~\ref{fig:graph_gen_pipeline}). The descriptions split the dynamic situations by diverse activity moments, and $\{o_{i}\}$ and actions $\{a_{t}\}$ are associated with specific timestamps $\{y_{t}\}$.
Since the original descriptions are human-written text and typically without predefined formats, we utilize the LLMs to parse objects and actions from the description text into lists of them with appeared timestamps. 
We also employ a proposed \textit{goal} prompt $\omega$ to output the results in a unified \textit{format} $\phi$$\rangle$. 
% \bo{how to use the goal prompt, is the same goal as the goal in the next sentence?}
The \textit{format} shows the ideal output key-value lists (\eg, $\langle$[object: tofu, water, cornstarch, ...]$\rangle$ and $\langle$\{``action: ``cut tofu'', ``goal'': ``into square pieces''\}, ...$\rangle$). 
% \bo{check if it's correct or not for the action list}
Notably, some objects are observable in video frames but they were not annotated in the human text annotations. For those objects, we use BLIP2~\cite{} to identify objects $\{o_{i}^{*}\}$ in each frame $f_{t^{*}}$ and add them to the initial object list $\{o_{i}\}$.

\textbf{Attributes and Relationships.}
Then, we derive object attributes and object-object spatial relationships from sampled keyframes $\{f_{t^{*}}\}$ of video $v$. As depicted in 
Algorithm~\ref{algo:video_content_graph_generation}
, we request MiniGPT4~\cite{openai2023gpt} to response object attributes and object-object spatial relationships with a conversational process. \bo{need to highlight based on the details}
Through the prompts, the method generates various object attributes for visual, physical, and chemical properties and XX relationships (\eg, $\langle$\#Prompt\#: Please describe the tofu in the image in terms of size, shape, color, and texture in one short sentence within 10 words. \#Model\#: The tofus are small, white, sliced squares.$\rangle$). \bo{highlight the attribute selection reason for the given videos with an example; missing the relationship categories}


\textbf{Situated Knowledge Graph Extension}
% \bo{add: how to link or merge the relevant video content with the objects and acts} 
% \noindent\textbf{Merging Actions with Objects.} 
Lastly, we compare the timestamps of frames ${f_{t^{*}}}$ and actions $\{a_{t}\}$, as shown in Algorithm~\ref{algo:video_content_graph_generation}. If timestamp $t^{*}$ aligns with $t$ and object $o_{i}^{*}$ from $f_{t^{*}}$ appears in $a_{t}$ (\bo{Here, linking objects and actions via timestamps or linking the timestamps of objects by sub-obj actions?}), we add the corresponding edge representing \textit{(action, object)} to $\mbox{\boldmath$G$}_{v}$. Additionally, for each $a_{t}$, we include an edge representing \textit{(timestamp, action)} to indicate the sequence of actions.
The generation process is shown in the Algorithm of supplementary.
% ~\ref{algo:video_content_graph_generation}.
% \bo{Describe the graph construction based on the elements}
% We add edges representing \textit{(timestamp, object)}, \textit{(object, attribute)}, and \textit{(object$_{i}$, relation, object$_{j}$)} to $\mbox{\boldmath$G$}_{v}$. 

\subsection{General Knowledge Graph (GKG)}
\label{sec:method_general_knowledge_graph}

% \input{algorithms/alg2}  \bo{Move to supplementary}

% \bo{original version:}
% In the second stage, as shown in Algorithm~\ref{algo:general_knowledge_graph_generation}, we leverage an LLM to obtain the general knowledge of objects $\{o_{i}\}$ and actions $\{a_{t}\}$ in Video Content Graph. Then, to generate general knowledge of each object $o_{i}$ or action $a_{t}$, the prompt template is $\langle$\textit{general knowledge examples}, \textit{generation goal}, \textit{output format}$\rangle$ where \textit{general knowledge examples} correspond to a \textit{general knowledge aspect} and \textit{generation goal} is adjusted according to the aspect. Also, \textit{general knowledge examples} follow the \textit{output format} to guide the LLM to generate knowledge in the desired format.

% Using the video showing the cooking process of Mapo Tofu in Figure~\ref{fig:graph_gen_pipeline} as an example, for object \textit{cornstarch}, we instruct LLM to generate general knowledge in \textit{aspects} of \textit{physical}, \textit{chemical}, and \textit{usage}. The \textit{general knowledge examples} demonstrate the examples of knowledge in \textit{output format}.


% \bo{original version:}
% \textbf{
% For each object $o_{i}$ or action $a_{t}$, we utilize a prompt template: $\langle$\textit{general knowledge examples} $\pi$, \textit{generation goal} $\omega$, \textit{output format} $\phi$$\rangle$. The \textit{general knowledge examples} relate to a specific \textit{general knowledge aspect}, and the \textit{generation goal} is tailored based on the aspect.
% Furthermore, the \textit{general knowledge examples} adhere to an \textit{output format}, which directs the LLM by in-context learning to generate knowledge in the desired format.
% We demonstrate this process using the video depicting the cooking process of Mapo Tofu in Figure~\ref{fig:graph_gen_pipeline}. For instance, when addressing the object \textit{cornstarch}, we instruct the LLM to generate general knowledge encompassing the \textit{aspects} of \textit{physical}, \textit{chemical}, and \textit{usage}. The \textit{general knowledge examples} provide illustrations of knowledge in the specified \textit{output format}. This generated knowledge is then linked to the corresponding aspect and object \textit{cornstarch} through edges added to the General Knowledge Graph $\mbox{\boldmath$G$}_{gk}$. A similar process is applied to other objects and actions.
% }

\textbf{General Knowledge Prompt.}
The relevant general knowledge covers the multiple perspectives of knowledge domains including \textit{usage}, \textit{physical}, \textit{chemical}, and \textit{culture}, etc. \bo{introduce all the adopted aspects here}
For instance, when addressing the object \textit{cornstarch} during a dish cooking process, we hope to cover general knowledge encompassing the \textit{aspects} of \textit{physical}, \textit{chemical}, and \textit{usage}. 


Suppose we want to generate useful general knowledge of ``tofu'' (a Chinese food product prepared by coagulating soy milk and then pressing the resulting curds into solid white blocks of varying softness\cite{XX}). A naive and straightforward way is asking the LLM ``Tell me some common knowledge about tofu'' (only have ``generation goal''), then the LLM can generate some relevant knowledge descriptions. However, the generated text is uncontrollable without specific content key points. For example, the LLM does not tell us the color of tofu. Thus, we denote the aspects (\eg, physical, cultural) for knowledge generation and collaborate with ``goal'' to make it more specific.

Meanwhile, we also hope to generate content in desired formats, because keeping the generation specificity is not always enough. 
Because LLM outputs can be wordy, unstructured, or there exists repeated content, such as `` Tofu is a popular food ...'' or ``Tofu is a versatile ingredient that ...''.
(\bo{give a negative example}). 
We use \textit{general knowledge examples} to adhere to an \textit{output format}, which leverages the in-context learning capacity of the LLM to generate new knowledge information in a predefined desired format. To be efficient, we need to limit the content length. 
Therefore, we add ``output format'' to guide LLM to output in JSON format and limit the content length. 
Then, we find LLM may output invalid JSON format if we directly ask it to output in JSON format like this: $\langle$\{``tofu'': ...\{``physical'': ``color'': ``white\}\}$\rangle$. There is a missing quotation mark of the word white. The whole content cannot be parsed in JSON format. So we finally provide examples of knowledge in JSON format to guide LLM. The output token amount will also be less.

\begin{figure*}[t]
  %\setlength{\abovecaptionskip}{0pt}
  %\setlength{\belowcaptionskip}{0pt}
  \centering
  \includegraphics[width=18cm]{figures/fig_graph_gen_pipeline.pdf}
  \caption{Generation pipeline of Video Content Graph (VG, see Section~\ref{sec:method_situated_knowledge_graph}), General Knowledge Graph (GKG, see Section~\ref{sec:method_general_knowledge_graph}), and Situated Knowledge Graph (SKG, see Section~\ref{sec:method_situated_commonsense_knowledge_graph}).}
\label{fig:graph_gen_pipeline}
\end{figure*}

\textbf{General Knowledge Graph Construction.}
As illustrated in Algorithm~\ref{algo:general_knowledge_graph_generation}, we employ an LLM to acquire general knowledge about objects $\{o_{i}\}$ and actions $\{a_{t}\}$ presented in dynamic situations.
% For each object $o_{i}$ or action $a_{t}$, 
We collect and construct the general knowledge beginning from the object $o_{i}$ or action $a_{t}$ as initial nodes. To represent multi-hop knowledge for various aspects, each node is desirable to have associated edges. 
We adopt multiple rounds of conversations to generate a graph by extending the object or action nodes with new nodes or paths. For each step of generation, we design a prompt with the triplet: $\langle$\textit{general knowledge examples} $\pi$, \textit{generation goal} $\omega$, \textit{output format} $\phi$$\rangle$. The \textit{generation goal} relates to a specific aspect of commonsense knowledge, and the \textit{general knowledge examples} is tailored based on the aspect.
Here is an exemplary output for the 5 usages of cornstarch: [\{"sauce": "thickening"\}, \{"batter": "making crispy"\}, \{"body powder": "absorbing moisture"\}, \{"starch": "making"\}, \{"playdough": "creating homemade"\}]



% \bo{need to add}

% ==========

% highlight points:

% Why we need ``GK examples'', ``Generation goal'', and ``Output format'' to generate high quality general knowledge in desired format.

% 1. Suppose we want to generate general knowledge of ``tofu''. The naive way is asking LLM ``Tell me some commonsense knowledge about tofu'' (only have ``Generation goal''). The LLM can generate some knowledge. However, the content is totally uncontrollable and unstructured. And the generated knowledge can be wordy and there exists repeated content, such as `` Tofu is a popular food ...'' and ``Tofu is a versatile ingredient that ...''.

% 2. Therefore, we add knowledge aspect (\eg, physical, cultural) to ``Generation goal'' to make it more specific

% 3. But specificity is not enough. To generate GKG, we need the generated content in desired format. And LLM can be wordy. To be efficient, we need to limit the content length. Therefore, we add ``Output format'' to guide LLM to output in JSON format and limit the content length.

% 4. However, we find LLM may output ``wrong'' JSON format if we directly ask it to output in JSON format. (LLM's output is pure string. We need to convert the string to dict or list). LLM may output something like this $\langle$\{``tofu'': ...\{``physical'': ``color'': ``white\}\}$\rangle$. There is a missing quotation marks of word white. The whole content cannot be parsed in JSON format. Therefore, we need examples of knowledge in JSON format to guide LLM. The token used will also be less.

% ==========

% For example,Fig~\ref{fig:graph_gen_pipeline}) or 
% ``tofu'':
% \{
% ``physical'': \{``texture'': ``soft and smooth'', ``shape'': ``block or curd-like'', ... \},
% ``composition'': \{``main ingredient'': ``soybeans'', ``coagulant'': ``calcium sulfate or magnesium chloride'' \},
% ... \}

% Andong: example of GKG generation, object usage

% INPUT:

% \#System\#: You are a knowledgeable assistant. You know a lot about object usages.

% \#User\#: Please tell me 5 usages of water. The answer should be short and precise following the format '\textless{}the thing applied on\textgreater{}: \textless{}how to apply\textgreater{}'. The answer is a list in simple JSON format where each item is a dict and the key is \textless{}the thing applied on\textgreater{}.

% \#Assistant\#: [\{"human": "hydration"\}, \{"dirt": "cleaning"\}, \{"food": "cooking"\}, \{"crop": "irrigation"\}, \{"electricity": "power generation"\}].

% \#User\#: Please tell me 5 usages of salt. The answer should be short and precise following the format '\textless{}the thing applied on\textgreater{}: \textless{}how to apply\textgreater{}'. The answer is a list in simple JSON format where each item is a dict and the key is \textless{}the thing applied on\textgreater{}.

% \#Assistant\#: [\{"food": "preserving"\}, \{"stained coffee mugs": "cleaning"\}, \{"clothes": "removing stains from"\}, \{"grease fires": "extinguishing"\}, \{"cutting boards": "refreshing"\}],

% \#User\#: Please tell me 5 usages for cornstarch. The answer should be short and precise following the format '\textless{}the thing applied on\textgreater{}: \textless{}how to apply\textgreater{}'. The answer is a list in simple JSON format where each item is a dict and the key is \textless{}the thing applied on\textgreater{}.

% OUTPUT:

% \#Assistant\#: [\{"sauce": "thickening"\}, \{"batter": "making crispy"\}, \{"body powder": "absorbing moisture"\}, \{"starch": "making"\}, \{"playdough": "creating homemade"\}]


\subsection{Situated Commonsense Knowledge Graph (SCKG)}
\label{sec:method_situated_commonsense_knowledge_graph}
% \input{algorithms/alg3}

% We generate Situated Knowledge Graph $\mbox{\boldmath$G$}_{sk}$ by combining Video Content Graph $\mbox{\boldmath$G$}_{v}$ and General Knowledge Graph $\mbox{\boldmath$G$}_{gk}$ as demonstrated in Algorithm~\ref{algo:situated_commonsense_knowledge_graph_generation}. For each object $o_{i}$ and each action $a_{t}$, we instruct LLM to analyze their functions and their logical relationships with others to generate situated knowledge. The prompt template is: $\langle$\textit{video content} $g_{v}$, \textit{general knowledge} $k_{g}$, \textit{situated knowledge examples} $\pi$, \textit{generation goal} $\omega$, \textit{output format} $\phi$$\rangle$. The \textit{video content} is a textualized version of $\mbox{\boldmath$G$}_{v}$ and \textit{general knowledge} corresponds to the select object $o_{i}$ or action $a_{t}$. Similar to the \textit{general knowledge examples} for $\mbox{\boldmath$G$}_{gk}$, \textit{situated knowledge examples} relate to a \textit{situated knowledge aspect} (\eg, \textit{counterfactual} and \textit{purpose}). However, as shown in Algorithm~\ref{algo:situated_commonsense_knowledge_graph_generation}, we do not provide the examples manually in advance but propose our \textbf{Self-Few-Shot Prompting} technique by utilizing former generated situated knowledge as examples.

% \bo{rephrased:}
Commonsense knowledge differs from encyclopedic knowledge in that it deals with general knowledge rather than the details of specific entities~\cite{tandon2018}.
In our work, Situated Commonsense Knowledge Graph $\mbox{\boldmath$G$}_{sk}$ is a generated novel knowledge graph conditioned on Situated Knowledge Graph $\mbox{\boldmath$G$}_{v}$ and General Knowledge Graph $\mbox{\boldmath$G$}_{gk}$ of the same dynamic situation. 
For each node (object $o_{i}$ or action $a_{t}$), we apply the relevant general knowledge from GKG to analyze their roles and logical relationships within the given situation represented by SKG.
Here, we illustrate the importance and complexity of generating situated commonsense knowledge through a simple example. Let's consider a counterfactual scenario where we want to ask about the effects of not using cornstarch in the preparation of mapo tofu (as demonstrated in Figure~\ref{fig:graph_gen_pipeline}). Relying solely on situated knowledge in the VG or general knowledge of cornstarch in GKG, then directly extracting the information (\ie, it is a powdery substance), would not provide us with the correct answer. Instead, we need to leverage the situated knowledge about cornstarch from SKG (\eg, ``The person mixes cornstarch with water and adds the mixture to the soup.'') and integrate it with relevant general knowledge from GKG (\eg, ``Cornstarch can be used as a thickening agent.'') to deduce the consequences of not using cornstarch. The result for the example would be ``The sauce would lack thickness and the dish would have a thinner consistency.''.

% We link the knowledge descriptions to generate situated knowledge graphs via causal or relevant relations.

% \subsubsection{Situated Knowledge Generation via Few-Shot Self-Prompting}
% \noindent\textbf{Self-Few-Shot Prompting for Concrete and Specific Knowledge Generation.} The need for this technique is that we find, without examples, the LLM may generate situated knowledge that is semantically correct but less concrete and specific. For instance, without examples, if we ask LLM with \textit{generation goal}: ``What would happen if the person did not use ground pork during cooking mapo tofu?'' with \textit{output format}: ``The answer should be short, precise, and specific'', the model may still answer ``The dish would lack flavor and texture'', which is correct but too general and not ``situated'' enough. However, we cannot manually provide examples in advance to instruct LLM how ``specific'' the generated knowledge should be as the knowledge is situated on video $v$. To tackle the problem, as shown in Algorithm~\ref{algo:situated_commonsense_knowledge_graph_generation}, we use the generated situated knowledge of other objects or actions as examples. We repeat the whole process in multiple iterations and update the knowledge in the examples. For instance, the consequence of not using ground pork answered by LLM would finally be ``The dish would lack meaty flavor, texture, and richness.''

Intuitively, the prompt of situated commonsense knowledge generation could be a quadruple: $\langle$\textit{video content} $g_{v}$, \textit{general knowledge} $k_{g}$, \textit{generation goal} $\omega$, \textit{output format} $\phi$$\rangle$. However, our experiments discover that LLM may generate situated commonsense knowledge that is semantically correct but lacks concrete and specific representations. For instance, although we query the LLM with a \textit{generation goal} and an \textit{output format} stating (such as, ``What would happen if the person did not use ground pork during cooking mapo tofu?'' and ``The answer should be short, precise, and specific''), the model may still respond with ``The dish would lack flavor and texture.'' While this answer is correct, it is too general and irrelevant to situated conditions.
Meanwhile, it is not feasible to manually provide examples in advance to instruct the LLM on the desired level of specificity, as the knowledge is situated on video $v$. 
Therefore, we propose a method called Few-Shot Self-Prompting to tackle the problem.

\textbf{Few-Shot Self-Prompting.} Few-shot self-prompting leverages previously generated situated commonsense knowledge as examples, as demonstrated in Algorithm~\ref{algo:situated_commonsense_knowledge_graph_generation}.  In this approach, the prompt comprises a pentad: $\langle$\textit{video content} $g_{v}$, \textit{general knowledge} $k_{g}$, \textit{situated commonsense knowledge examples} $\pi$, \textit{generation goal} $\omega$, \textit{output format} $\phi$$\rangle$.

As illustrated in Figure~\ref{fig:graph_gen_pipeline}, the \textit{situated knowledge examples} $\pi$ are constructed using previously generated knowledge concerning the consequences of not using a specific ingredient (in this case, only ``cornstarch'' is shown due to content limitations in Figure~\ref{fig:graph_gen_pipeline}). The newly generated knowledge is then added to the \textit{situated commonsense knowledge examples}. Over time, this process results in increasingly concrete and specific situated commonsense knowledge. We demonstrate the final generation results: the consequence if not using ground pork would be ``The dish would lack meaty flavor, texture, and richness, resulting in a vegetarian version of mapo tofu.'' The intuition of the proposed Few-Shot Self-Prompting technique might be that the knowledge of other objects or actions can serve as a contrast to the current one. Leveraging the model's in-context learning ability can generate more concrete and specific knowledge about the target object or action.

Using our Few-Shot Self-Prompting technique, we employ a selection of situated commonsense knowledge perspectives. These include the ability to consider \textit{counterfactual} scenarios for an object or action, understand the \textit{purpose of an action} within a given situation, and recognize the \textit{contribution of an object} to the process (represented as $\{\eta_{i}^{obj}\}$, $\{\eta_{i}^{act}\}$
% in Algorithm~\ref{algo:situated_commonsense_knowledge_graph_generation}
). Notably, our experimental findings indicate that even just two iterations of knowledge generation yield high-quality knowledge outcomes. Ultimately, this process culminates in the acquisition of a SCKG $\mbox{\boldmath$G$}_{sk}$.

% Here, we do not provide the examples manually beforehand, so the approach improves the efficiency of the method and allows for a more streamlined generation of the Situated Knowledge Graph.
% The motivation is that we find, without examples, that the LLM may generate situated knowledge that is semantically correct but less concrete and specific. For instance, without examples, if we query the LLM with a \textit{generation goal} such as, "What would happen if the person did not use ground pork during cooking mapo tofu?" and an \textit{output format} stating, "The answer should be short, precise, and specific," the model may still respond with "The dish would lack flavor and texture." While this answer is correct, it is too general and insufficiently "situated."
% However, it is not feasible to manually provide examples in advance to instruct the LLM on the desired level of specificity, as the knowledge is situated on video $v$. 
% \bo{check if duplicate with the above description:}


% \textbf{Situated Commonsense Knowledge Generation.}
% \bo{present how to generate aligned knowledge?}

% \bo{original version: Are there any highlight points during the generation prompt design or process?}

% % as illustrated in Algorithm~\ref{algo:situated_commonsense_knowledge_graph_generation}, 
% To address this challenge, we utilize the generated situated knowledge of other objects or actions as examples. We repeat the entire process in multiple iterations, updating the knowledge in the examples accordingly. For example, the consequence of not using ground pork, as answered by the LLM, would ultimately be, "The dish would lack meaty flavor, texture, and richness, resulting in a vegetarian version of mapo tofu."

% \bo{why and how to generate situated commonsense knowledge}
% The prompt template is defined as: $\langle$\textit{video content} $g_{v}$, \textit{general knowledge} $k_{g}$, \textit{situated knowledge examples} $\pi$, \textit{generation goal} $\omega$, \textit{output format} $\phi$$\rangle$. The \textit{video content} is a textual representation of $\mathbf{G}_{v}$, and the \textit{general knowledge} corresponds to the selected object $o_{i}$ or action $a_{t}$. Similar to the \textit{general knowledge examples} for $\mathbf{G}_{gk}$, the \textit{situated knowledge examples} are associated with a \textit{situated knowledge aspect} (\eg, \textit{counterfactual} and \textit{purpose}).


% ==========

% highlight points:

% why we need each prompt component

% 1. The naive way, only having ``Video content'' (to make the knowledge situated) and ``Generation goal''. We may get wordy and non-specific knowledge.

% 2. The reason of having ``Output format'' is similar to GKG

% 3. However, with ``Video content'' + ``Generation goal'' + ``Output format'', the generated knowledge is not specific and concrete enough. Therefore, we add self few shot prompting (``SK examples'') is shown in Sec 3.3

% 4. However, still, the generated knowledge can be situated but may miss some points. We provide ``General knowledge'' explicitly in prompt design to guide the LLM. For example, without ``General knowledge'', asking LLM ``Why using cornstarch'', the model could answer ``Thickening the soup''. With ``General knowledge'' which shows the usges of cornstarch include ``thickening agent'' and ``coating and frying'', now model will answer ``Thickening the soup and coating tofu''.

% ==========


% ==========
% Andong; example of SKG generation, object, counterfactual

% \#System\#: You are a helpful, pattern-following assistant. You are very good at deciphering a video, such as summarizing video content, figuring out related commonsense knowledge, and identifying the inner logic. As a commonsense-driven assistant, your task is to analyze a video (length: 119 seconds) that showcases a person introducing 6 cooking steps of mapo tofu.

% The steps are described in a specific format of '[Step N (from <timestamp> to <timestamp>): detailed description of cooking actions]' as follows: [Step 1 (from <16 sec> to <30 sec>): cut tofu into square pieces] ...

% Objects appeared in different frames are described in a specific format of '[Objects at <timestamp>: object(s): attributes of objects]' or '[Objects from <timestamp> to <timestamp>: object(s): attributes of objects]' as follows: [Objects at <0 sec>: tofu: small, square, creamy tofu.] ...

% The relationship of objects are in different frames in format of ‘[object 1 and object 2 at <timestamp>: relationship]’: [tofu and knife at <21 sec>: knife cuts tofu into small squares.] ... 

% The background knowledge of objects appeared in the video is:
% 'cornstarch':{ 'physical': {'state': 'powder', 'color': 'white', ...

% BEFORE:

% \#User\#: What would happen if the person did not use ground pork during cooking mapo tofu? The answer should be direct, precise, short, and within 20 words in one sentence without any comma. Word 'ground pork' should not be included in the answer.

% \#Assistant\#: The dish would lack flavor and texture.

% AFTER

% \#User\#: What would happen if the person did not use water during cooking mapo tofu? The answer should be direct, precise and short and within 20 words in one sentence without any comma. Word 'water' should not be included in the answer.

% \#Assistant\#: The dish would lack moisture, resulting in a dry and less saucy version of mapo tofu.

% \#User\#: What would happen if the person did not use mapo tofu paste during cooking mapo tofu? The answer should be direct, precise and short and within 20 words in one sentence without any comma. Word 'mapo tofu paste' should not be included in the answer.

% \#Assistant\#: The dish would lose its signature flavor and spiciness, resulting in a dish that is not mapo tofu.

% \#User\#: What would happen if the person did not use ground pork during cooking mapo tofu? The answer should be direct, precise and short and within 20 words in one sentence without any comma. Word 'ground pork' should not be included in the answer.

% \#Assistant\#: The dish would lack meaty flavor, texture, and richness, resulting in a vegetarian version of mapo tofu.

% ==========

\subsection{Question and Answer Generation}
\label{sec:method_qa_gen}

Utilizing the Situated Knowledge Graph (SKG), General Knowledge Graph (GKG), and Situated Commonsense Knowledge Graph (SCKG) mentioned above, we generate question-answer pairs to assess the model's capability to make accurate inferences. This evaluation process leverages both factual information specific to a given situation and the essential commonsense knowledge required. To accomplish this, we can adopt two approaches: \textbf{(1)} Manual question-answer templates in a bottom-up manner, where we design question templates and provide corresponding answers based on the graphs. \textbf{(2)} Automatic question generation by utilizing a LLM in a top-down manner.

% Based on the above three graphs, Situated Knowledge Graph (SKG), General Knowledge Graph (GKG), and Situated Commonsense Knowledge Graph (SCKG), we generate question-answer pairs to evaluate the model’s ability to make appropriate inferences by taking advantage of both factual information within a given scenario and the necessary commonsense knowledge. We can achieve this by either manual question-answer templates in a bottom-up manner or automatic question generation by leveraging an LLM in a top-down manner.

\begin{table}[h]
    % \setlength{\abovecaptionskip}{0pt}
    % \setlength{\belowcaptionskip}{0pt}
    \caption{Question template types for Bottom-up QA generation}
    %\tiny %\scriptsize
    \footnotesize
    \centering
    \begin{threeparttable}
    \begin{tabular}{ll}
    \toprule
    % \multicolumn{2}{l}{Reasoning   types} \\
    % \cmidrule(lr){1-2}
    \textbf{Object counterfactual} & vanilla (obj) \\
    (\eg, What would happen if & + obj attributes \\
    the person did not use…) & + obj-obj relationships \\
     & + obj attribute + obj-obj relationship \\
     & + obj general knowledge \\
    \cmidrule(lr){1-2}
    \textbf{Object contribution} & vanilla (obj) \\
    (\eg, Why the person & + obj attributes \\
    use...) & + obj-obj relationships \\
     & + obj attribute + obj-obj relationship \\
     & + obj general knowledge \\
    \cmidrule(lr){1-2}
    \multicolumn{2}{l}{\textbf{Object reasoning}} \\
    \multicolumn{2}{l}{(\eg, What are the two objects which \textless{}interaction\textgreater{})} \\
    \cmidrule(lr){1-2}
    \textbf{Action counterfactual} & vanilla (act) \\
    (\eg, What would happen if & + before / after action \\
    the person did not…) & + before / after action + obj attr / rela \\
    \cmidrule(lr){1-2}
    \textbf{Action purpose} & vanilla (act) \\
    (\eg, Why the person...) & + before/after action \\
     & + before / after action + obj attr / rela \\
    \cmidrule(lr){1-2}
    \multicolumn{2}{l}{\textbf{Action possibility}} \\
    \multicolumn{2}{l}{(\eg, What mistake might the person make if \textless{}possibility\textgreater{})} \\ %\rowcolor{gray!20} 
    \bottomrule
    \end{tabular}
    % \begin{tablenotes}
    % \footnotesize
    % \item 
    % \end{tablenotes}
    \end{threeparttable}
    \label{tab:method_ques_templates}
\end{table}

\subsubsection{Bottom-up QA Generation}
\label{sec:method_rule_based_qa_gen}

We manually design question templates in multi hog way combing both ``situation'' and ``commonsense'' (see the template types in Table~\ref{tab:method_ques_templates}). For one object / action, we find the connected edges in the three graphs. Next, we design question templates that jump from edges in Situated Knowledge Graph or General Knowledge Graph to those in Situated Commonsense Knowledge Graph. Concretely, for example, the template of question type ``obj counterfactual + obj attribute + obj-obj relation'' as illustrated in Table~\ref{tab:method_ques_templates} would be ``What would happen if the person did not use the \textit{\textless{}obj attribute\textgreater{}} and \textit{\textless{}obj-obj relation\textgreater{}}?''. You can see the specific question example concerning ``cornstarch'' in Figure~\ref{fig:teaser}. The model needs to first do spatiotemporal reasoning to identify the object by  \textit{\textless{}obj attribute\textgreater{}} and \textit{\textless{}obj-obj relation\textgreater{}} (\eg, ``white substance'' and ``dissolved in water in glass''). Next, the model needs to do situated commonsense reasoning to understand the consequence if that object was not used. In such way, we can comprehensively test model's situated commonsense reasoning ability. Note that we also present some easier templates (\eg, ``vanilla obj counterfactual'') which are single hog.

% We design question templates to reflect the diverse task types and the specific question key points.
% According to the edges from VG and GKG with those from SKG, the template is able to compose both elementary components within the situations and reasoning logics for questions. 
% For instance, for question type ``object counterfactual + obj attribute + obj-obj relationship'' as illustrated in Table~\ref{tab:method_ques_templates}, we select edges that signify \textit{object attributes} and \textit{object-object relationships} from VG. Subsequently, for the same \textit{object}, we choose edges that represent the \textit{counterfactual} situations about an \textit{object} from SKG. By merging these edges and utilizing the corresponding question template (for the question type, the template can be ``What would happen if the person did not use the \textit{\textless{}obj attribute\textgreater{}} object \textit{\textless{}obj-obj relationship\textgreater{}}?''), we can generate questions as demonstrated in Figure~\ref{fig:question_examples}. These templates enable the generated questions to assess the model's spatiotemporal and commonsense reasoning capabilities within a given context.

\subsubsection{Top-down QA Generation}
\label{sec:method_top_down_qa_gen}

Bottom-up QA generation offers control over question quality and difficulty but lacks flexibility in creating diverse question types. To overcome this limitation, we suggest a top-down approach for QA generation. We design a structured prompt $\langle$\textit{video content}, \textit{integrated graph}, \textit{QA examples}, \textit{generation goal}, \textit{output format}$\rangle$. The \textit{integrated graph} combines SKG, GKG, and SCKG. \textit{QA examples} are randomly selected from bottom-up generated QAs, while the \textit{generation goal} instructs the LLM to create multi-hop questions based on multiple edges from \textit{integrated graph}. This prompt design maintains a strong connection between the generated QAs and graphs, significantly reducing the likelihood of model hallucination when compared to basing QAs solely on video content.

However, the top-down approach has its drawbacks—it is resource-intensive and slow. With the three graphs involved, top-down QA generation takes a few seconds to generate one question, whereas the bottom-up method generates the entire benchmark in the same time. In this paper, we primarily use the bottom-up method for creating the benchmark, but we discuss top-down generation case studies in the Supplementary Material.

% \subsubsection{question-answer and graphs}
% \label{sec:method_qa_graph_alignment}

% ==========

% example of rationale

% Q: What would happen if the person did not use the white substance dissolved in water in glass?

% Choices:

% A. The dish would be completely different.

% B. The dish would lack thickening agent. (correct)

% C. The dish would lack seasoning and taste bland.

% D. The dish would lose its signature flavor.

% Reasoning process generated by LLM

% 1. From [object attributes], we can see that cornstarch is white.

% 2. From [object-object relations], we can see that cornstarch is dissolved in water in glass.

% 3. In the video, Step 2 (from 32 sec to 40 sec): put cornstarch in a small bowl and mix with water

% 4. Step 6 (from 98 sec to 105 sec): add cornstarch and stir gently

% 5. From [General Knowledge Graph], we know that cornstarch can be used as thickening agent to thicken soups.

% 6. From the video, from 32 sec to 40 sec, we can see that cornstarch is put in a small bowl and mixed with water to form a paste.

% 7. This paste is then added to the dish (from 98 sec to 105 sec) to thicken the sauce.

% 8. Therefore, the correct answer is The dish would lack thickening agent.

% 9. The other choices can be eliminated because they are not the correct consequences if the person did not use cornstarch.

% ==========
\subsubsection{Data Source}
We created the benchmark based on videos of the two public video datasets about daily activities, as detailed in Table~\ref{tab:dataset_sources_youcook2_homage}. They have high-quality videos and captions, and the videos exhibit entities and logical relationships between actions. 
% YouCook2~\cite{zhou2018towards} and HOMAGE~\cite{rai2021home}

\begin{table}[t]
    \setlength{\abovecaptionskip}{0pt}
    \setlength{\belowcaptionskip}{0pt}
    \caption{Video Data Source}
    %\tiny %\scriptsize
    \scriptsize
    \centering
    \begin{threeparttable}
    \begin{tabular}{p{1.2cm}C{1cm}C{0.5cm}C{0.5cm}C{0.1cm}C{0.1cm}C{0.6cm}C{0.6cm}}
    \toprule
    Data Source & \multicolumn{3}{c}{Content} & \multicolumn{4}{c}{Annotation} \\
     & Obj & Act & Scene & Obj & Act & Temporal & Relations \\
    \cmidrule(lr){2-4}\cmidrule(lr){5-8}
    HOMAGE~\cite{rai2021home} & daily & daily & home & \checkmark & \checkmark & \checkmark & \checkmark \\
    YouCook2~\cite{zhou2018towards} & ingredients & cooking & kitchen & \checkmark & \checkmark & \checkmark &  \\
    \bottomrule
    \end{tabular}
    % \begin{tablenotes}
    % \footnotesize
    % \item 
    % \end{tablenotes}
    \end{threeparttable}
    \label{tab:dataset_sources_youcook2_homage}
\end{table}


\noindent\textbf{YouCook2}~\cite{zhou2018towards} is a comprehensive collection of instructional cooking videos from YouTube. It features over 2,000 videos, spanning 89 different recipe categories, where each video is annotated with detailed step-by-step instructions.

\noindent\textbf{HOMAGE}~\cite{rai2021home} consists of 1,752 video clips including 75 human daily activities within home environments. The dataset is richly annotated with action labels, object information, and spatial-temporal relationships.

\subsection{Quality Valiation}
We invite human helpers to manually assess the quality of the graphs and QAs. Please see Supplementary Material for more details.

% You must include your signed IEEE copyright release form when you submit your finished paper.
% We MUST have this form before your paper can be published in the proceedings.

% Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
% \url{https://www.computer.org/about/contact}.





























% \newpage
\section{Situated Commonsense Reasoning \\ Benchmark}
\label{sec:benchmark}

\begin{figure*}[h]
  %\setlength{\abovecaptionskip}{0pt}
  %\setlength{\belowcaptionskip}{0pt}
  \centering
  \includegraphics[width=18cm]{figures/fig_qa_examples.pdf}
  \caption{Examples of generated question-answer pairs of the benchmark. We demonstrate associated graphs to the QA pairs.}
\label{fig:qa_examples}
\end{figure*}

\subsection{Benchmark Overview}
Our benchmark consists of 44K questions and answers for reasoning with situated open-world knowledge, accompanied by multiple-choice options, and 10K video clips. Each question-answer (QA) pair links to a hypergraph, as illustrated in Figure~\ref{fig:teaser}. These hypergraphs are sampled from larger graphs called Situated Knowledge Graph (see Section~\ref{sec:method_situated_knowledge_graph}), General Knowledge Graph (see Section~\ref{sec:method_general_knowledge_graph}), and Situated Commonsense Knowledge Graph (see Section~\ref{sec:method_situated_commonsense_knowledge_graph}). The alignment of hypergraphs with question-answer pairs effectively demonstrates the structured abstraction of video situations and situated knowledge. In addition to the hypergraphs, we provide a rationale that illustrates the reasoning steps taken from the question to the answer (see Figure~\ref{fig:teaser}).
There are 12 types of questions shown in Figure~\ref{fig:dataset_stat}.
% Notably, the ``Spatiotemporal (ST)'' includes ``obj attributes'', ``obj-obj relations'', ``obj attribute + obj-obj relation'', and ``before/after action'' (see details in Section~\ref{sec:method_qa_gen}).
% ``General knowledge (GK)'' covers aspects such as ``physical'', ``chemical'', ``cultural'', and ``usage''.
For each question, we provide two answer formats: a direct answer and a multiple-choice format with four options. As seen in Figure~\ref{fig:dataset_stat}, the distribution of these choices is debiased. Additionally, we utilize LLM to detect and correct any grammatical errors in the questions.

% For each question, we provide two answer formats: a direct answer and a multiple-choice format with four options. One option is annotated as the correct choice, while the other three incorrect options are randomly selected from the same knowledge aspect, but related to different objects or actions. Furthermore, we associate each question-answer pair with a corresponding video clip from the raw video, based on the objects and actions mentioned in the text.

\begin{figure}[t]
  %\setlength{\abovecaptionskip}{0pt}
  %\setlength{\belowcaptionskip}{0pt}
  \centering
  \includegraphics[width=8.5cm]{figures/fig_dataset_stat.pdf}
  \caption{\textbf{(a)} Sankey diagram of the 12 question types. \textbf{(b)} Answer distribution among options for each question type. Meaning of abbreviations: O: Object; A: Action; CT: Counterfactual; CB: Contribution; PU: Purpose; R: Reasoning; PO: Possibility; ST: Spatiotemporal; GK: General knowledge. Notably, the ``Spatiotemporal'' includes ``obj attributes'', ``obj-obj relations'', ``obj attribute + obj-obj relation'', and ``before/after action'' (see Section~\ref{sec:method_qa_gen}).}
\label{fig:dataset_stat}
\end{figure}


\subsection{Benchmark Generation}
We introduce a novel method to efficiently create the benchmark in a controllable and structured manner. If a person were to manually create this benchmark, it would involve four implicit stages: 1) parsing the content of situations, \ie, what can be directly observed in the video; 2) listing related commonsense knowledge as comprehensively as possible; 3) applying reasoning abilities to align situation content components with commonsense knowledge, thereby uncovering hidden logical connections and potential consequences; 4) composing questions and providing answers by synthesizing the aforementioned information.

To enhance the efficiency and structure of this process, we replace human annotators with a Large Language Model (LLM). We design a series of prompt templates that instruct LLM to generate three essential components corresponding to the first three stages: 1) Situated Knowledge Graph (SKG, see Section~\ref{sec:method_situated_knowledge_graph}); 2) General Knowledge Graph (GKG, see Section~\ref{sec:method_general_knowledge_graph}); and 3) Situated Commonsense Knowledge Graph (SCKG, see Section~\ref{sec:method_situated_commonsense_knowledge_graph}).

In correspondence with the final stage, we can leverage these graphs to either manually construct question templates (Section~\ref{sec:method_rule_based_qa_gen}) or instruct the LLM (Section~\ref{sec:method_top_down_qa_gen}) to generate question-answer pairs (QAs). This approach enables a clear alignment between the generated QAs and the graphs and corresponding rationale indicating reasoning steps from Q to A. Further details on our generation method are presented in the following sections.

% Lastly, We evaluate the quality of the graphs and QAs through manual assessment.

% Suppose a person manually creates this benchmark, there would be three stages: 1) the person first parses situation content (\ie, what the person can directly see in the video). 2) Next, the person list related commonsense knowledge as much as possible. 3) Finally, the person uses his or her reasoning ability to align the situation content components with commonsense knowledge to reveal hidden logic (\eg, the consequences if an action did not take place). In our study, to make the whole process more effective and in a more structured way, we replace the person with LLM. Corresponding, we design a series of prompt templates to instruct LLM to generate 1) Video Content Graph (VG, see Section~\ref{}), 2) General Knowledgeable Graph (GKG, see Section~\ref{}), and 3) Situated Knowledge Graph (SKG, see Section~\ref{}). Based on the graphs, we may manually build question templates (Section~\ref{}) or instruct LLM (Section~\ref{}) to generate question-answer pairs (QAs). We can present a clear alignment between generated QAs and graphs. Finally, we assess the quality of the graphs and QAs manually.


\begin{figure*}[t]
  %\setlength{\abovecaptionskip}{0pt}
  %\setlength{\belowcaptionskip}{0pt}
  \centering
  \includegraphics[width=18cm]{figures/fig_graph_gen_pipeline.pdf}
  \caption{Generation pipeline of Video Content Graph (VG, see Section~\ref{sec:method_situated_knowledge_graph}), General Knowledge Graph (GKG, see Section~\ref{sec:method_general_knowledge_graph}), and Situated Knowledge Graph (SKG, see Section~\ref{sec:method_situated_commonsense_knowledge_graph}).}
\label{fig:graph_gen_pipeline}
\end{figure*}


\subsection{Situated Knowledge Graph (SKG)}
% \subsection{Video Content Graph (VG)}
\label{sec:method_situated_knowledge_graph}

% \input{algorithms/alg1} \bo{Move to supplementary}

% Original Version:
% Video Content Graph $\mbox{\boldmath$G$}_{v}$ describes what we can directly see in the video: objects, object attributes, object spatial relationships, actions, and action temporal relationships. There are three steps to construct the graph.

% It is important to note that we only use vision-language models to process objects, while relying on human annotations for actions, since current video-language models cannot accurately decipher action sequences from videos.

% We add edges representing \textit{(timestamp, object)}, \textit{(object, attribute)}, and \textit{(object$_{i}$, relation, object$_{j}$)} to $\mbox{\boldmath$G$}_{v}$. 
% \noindent\textbf{Merging Actions with Objects.} Finally, we compare the timestamps of frames ${f_{t^{*}}}$ and actions $\{a_{t}\}$ (see Algorithm~\ref{algo:video_content_graph_generation}). If timestamp $t^{*}$ aligns with $t$ and the object $o_{i}^{*}$ from $f_{t^{*}}$ appears in $a_{t}$, we add the corresponding edge which represents \textit{(action, object)} to $\mbox{\boldmath$G$}_{v}$. Also, for each $a_{t}$, we add the edge representing \textit{(timestamp, action)} to show the sequence of actions.

% \bo{rephrased}

Situated knowledge not only represents what is there but also describes the facts, effects, or dynamic processes of activities or events. We construct dynamic situations from videos, and they offer multi-frame event temporality, causality, and dynamics~\cite{buch2022}. 
Recently, more works have presented objects and relations by graphs in real-world dynamic situations~\cite{wu2021star,grunde2021agqa,urooj2023learning} and visual scenes~\cite{ji2020action,zellers2019recognition,hudson2019gqa}. 
 % $\mbox{\boldmath$G$}_{v}$
We extend visual graphs and propose a Situated Knowledge Graph with more visual entities and relations from dynamic situations: people/objects, attributes, relationships, or actions. 

% \textbf{Objects and Actions.}
We start from the object or action entity generation where they were labeled in the video descriptions from the source video dataset
% and associated with their appeared timestamps 
(\eg, shown in Figure~\ref{fig:graph_gen_pipeline}). 
The descriptions split the dynamic situations by diverse activity moments, and $\{o_{i}\}$ and actions $\{a_{t}\}$ are associated with specific timestamps $\{y_{t}\}$.
Since the original descriptions are human-written text and typically without predefined formats, we utilize the LLMs to parse objects and actions from the description text into lists of them with appeared timestamps. 
We employ a proposed \textit{format} 
% $\phi$$\rangle$ 
to output ideal formats: key-value lists.
% (\eg, $\langle$[object: tofu, water, cornstarch, ...]$\rangle$ and $\langle$\{``action: ``cut tofu'', ``goal'': ``into square pieces''\}, ...$\rangle$). 
% \bo{check if it's correct or not for the action list}
Notably, some objects are observable in video frames but they were not annotated in the human text annotations. 
For those objects, we use BLIP2~\cite{li2023blip} to identify objects in frames
and add them to the initial object list $\{o_{i}\}$.
% For those objects, we use BLIP2~\cite{li2023blip} to identify objects $\{o_{i}^{*}\}$ in each frame $f_{t^{*}}$ and add them to the initial object list $\{o_{i}\}$.

% \textbf{Attributes and Relationships.}
Then, object attributes and object-object spatial relationships are derived from sampled keyframes of videos.
% $\{f_{t^{*}}\}$ of video $v$. 
% As depicted in Algorithm~\ref{algo:video_content_graph_generation}, 
We request MiniGPT4~\cite{openai2023gpt} to response object attributes and object-object spatial relationships with a conversational process. 
% \bo{need to highlight based on the details}
Through the \textit{goal} prompt, the method generates various object attributes for visual, physical, and chemical properties and relationships (\eg, \#Prompt\#: Please describe the tofu in the image in terms of size, shape, color, and texture in one short sentence within 10 words. \#Model\#: The tofus are small, white, sliced squares.). 
% \bo{highlight the attribute selection reason for the given videos with an example; missing the relationship categories}


% \textbf{Situated Knowledge Graph Extension}
% \bo{add: how to link or merge the relevant video content with the objects and acts} 
% \noindent\textbf{Merging Actions with Objects.} 
% Lastly, we compare the timestamps of frames ${f_{t^{*}}}$ and actions $\{a_{t}\}$.
Lastly, we compare the timestamps of frames and actions.
% , as shown in Algorithm~\ref{algo:video_content_graph_generation}
% If timestamp $t^{*}$ aligns with $t$ and object $o_{i}^{*}$ from $f_{t^{*}}$ appears in $a_{t}$,
If the action timestamp matches the frame timestamps where objects appeared,
we add the corresponding edge representing \textit{(action, object)} to the situated knowledge graph. Additionally, for each action,
% $a_{t}$, 
we build an additional edge \textit{(timestamp, action)} to indicate the sequence of actions.
 % (\bo{Here, linking objects and actions via timestamps or linking the timestamps of objects by sub-obj actions?})
The generation process of SKG refers to the Algorithm of Supplementary Material.
% ~\ref{algo:video_content_graph_generation}.
% \bo{Describe the graph construction based on the elements}
% We add edges representing \textit{(timestamp, object)}, \textit{(object, attribute)}, and \textit{(object$_{i}$, relation, object$_{j}$)} to $\mbox{\boldmath$G$}_{v}$. 

\subsection{General Knowledge Graph (GKG)}
\label{sec:method_general_knowledge_graph}

% \input{algorithms/alg2}  \bo{Move to supplementary}

% original version:
% In the second stage, as shown in Algorithm~\ref{algo:general_knowledge_graph_generation}, we leverage an LLM to obtain the general knowledge of objects $\{o_{i}\}$ and actions $\{a_{t}\}$ in Video Content Graph. Then, to generate general knowledge of each object $o_{i}$ or action $a_{t}$, the prompt template is $\langle$\textit{general knowledge examples}, \textit{generation goal}, \textit{output format}$\rangle$ where \textit{general knowledge examples} correspond to a \textit{general knowledge aspect} and \textit{generation goal} is adjusted according to the aspect. Also, \textit{general knowledge examples} follow the \textit{output format} to guide the LLM to generate knowledge in the desired format.

% Using the video showing the cooking process of Mapo Tofu in Figure~\ref{fig:graph_gen_pipeline} as an example, for object \textit{cornstarch}, we instruct LLM to generate general knowledge in \textit{aspects} of \textit{physical}, \textit{chemical}, and \textit{usage}. The \textit{general knowledge examples} demonstrate the examples of knowledge in \textit{output format}.

% For each object $o_{i}$ or action $a_{t}$, we utilize a prompt template: $\langle$\textit{general knowledge examples} $\pi$, \textit{generation goal} $\omega$, \textit{output format} $\phi$$\rangle$. The \textit{general knowledge examples} relate to a specific \textit{general knowledge aspect}, and the \textit{generation goal} is tailored based on the aspect.
% Furthermore, the \textit{general knowledge examples} adhere to an \textit{output format}, which directs the LLM by in-context learning to generate knowledge in the desired format.
% We demonstrate this process using the video depicting the cooking process of Mapo Tofu in Figure~\ref{fig:graph_gen_pipeline}. For instance, when addressing the object \textit{cornstarch}, we instruct the LLM to generate general knowledge encompassing the \textit{aspects} of \textit{physical}, \textit{chemical}, and \textit{usage}. The \textit{general knowledge examples} provide illustrations of knowledge in the specified \textit{output format}. This generated knowledge is then linked to the corresponding aspect and object \textit{cornstarch} through edges added to the General Knowledge Graph $\mbox{\boldmath$G$}_{gk}$. A similar process is applied to other objects and actions.

% The relevant general knowledge covers the multiple perspectives of knowledge domains including \textit{usage}, \textit{physical}, \textit{chemical}, and \textit{culture}, etc.
% For instance, when addressing the object \textit{cornstarch} during a dish cooking process, we hope to cover general knowledge encompassing the \textit{aspects} of \textit{physical}, \textit{chemical}, and \textit{usage}.

% As illustrated in Algorithm~\ref{algo:general_knowledge_graph_generation}, we employ an LLM to acquire general knowledge about objects $\{o_{i}\}$ and actions $\{a_{t}\}$ presented in dynamic situations.
% % For each object $o_{i}$ or action $a_{t}$, 
% We collect and construct the general knowledge beginning from the object $o_{i}$ or action $a_{t}$ as initial nodes. To represent multi-hop knowledge for various aspects, each node is desirable to have associated edges. 
% We adopt multiple rounds of conversations to generate a graph by extending the object or action nodes with new nodes or paths. For each step of generation, we design a prompt with the triplet: $\langle$\textit{general knowledge examples} $\pi$, \textit{generation goal} $\omega$, \textit{output format} $\phi$$\rangle$. The \textit{generation goal} relates to a specific aspect of commonsense knowledge, and the \textit{general knowledge examples} is tailored based on the aspect.
% Here is an exemplary output for the 5 usages of cornstarch: [\{"sauce": "thickening"\}, \{"batter": "making crispy"\}, \{"body powder": "absorbing moisture"\}, \{"starch": "making"\}, \{"playdough": "creating homemade"\}]

We construct the general knowledge beginning from the object $o_{i}$ or action $a_{t}$ as initial nodes. Suppose we select ``tofu'' (a Chinese food product prepared by coagulating soy milk and then pressing the resulting curds into solid white blocks of varying softness). A naive and straightforward way is asking the LLM ``Tell me some common knowledge about tofu'' (only have ``generation goal''), then the LLM can generate some relevant knowledge descriptions. However, the generated text is uncontrollable without specific content key points. For example, the LLM does not tell us the color of tofu. Thus, we denote the aspects (\eg, \textit{usage}, \textit{physical}, \textit{chemical}, and \textit{culture}, etc) for knowledge generation and collaborate with ``goal'' to make it more specific.

We also aim to generate content in desired formats, as the LLM outputs can be verbose, unstructured, or contain repeated content, such as `` Tofu is a popular food ...'' or ``Tofu is a versatile ingredient that ...''. To address this issue, we employ \textit{general knowledge examples} to adhere to an \textit{output format}, which leverages the in-context learning capacity of the LLM to generate new knowledge information in a predefined desired format.

Relying solely on the \textit{output format} may still result in the LLM outputting invalid format (\eg, \{``tofu'': ...\{``physical'': ``color'': ``white\}\}, where there is a missing quotation mark for the word ``white'', resulting in JSON parsing failure.). By using both \textit{general knowledge examples} and \textit{output format}, we ensure the generated knowledge is of high quality and parseable as JSON.

Thus, as illustrated in Figure~\ref{fig:graph_gen_pipeline}, we utilize a prompt triplet $\langle$\textit{general knowledge examples} $\pi$, \textit{generation goal} $\omega$, \textit{output format} $\phi$$\rangle$ to guide the LLM. For instance, here is an example output for the 5 usages of cornstarch: [\{``sauce'': ``thickening''\}, \{``batter'': ``making crispy''\}, \{``body powder'': ``absorbing moisture''\}, \{``starch'': ``making''\}, \{``playdough'': ``creating homemade''\}]. Please see more details on GKG generation in the Algorithm of Supplementary Materials.

% ==========

% highlight points:

% Why we need ``GK examples'', ``Generation goal'', and ``Output format'' to generate high quality general knowledge in desired format.

% 1. Suppose we want to generate general knowledge of ``tofu''. The naive way is asking LLM ``Tell me some commonsense knowledge about tofu'' (only have ``Generation goal''). The LLM can generate some knowledge. However, the content is totally uncontrollable and unstructured. And the generated knowledge can be wordy and there exists repeated content, such as `` Tofu is a popular food ...'' and ``Tofu is a versatile ingredient that ...''.

% 2. Therefore, we add knowledge aspect (\eg, physical, cultural) to ``Generation goal'' to make it more specific

% 3. But specificity is not enough. To generate GKG, we need the generated content in desired format. And LLM can be wordy. To be efficient, we need to limit the content length. Therefore, we add ``Output format'' to guide LLM to output in JSON format and limit the content length.

% 4. However, we find LLM may output ``wrong'' JSON format if we directly ask it to output in JSON format. (LLM's output is pure string. We need to convert the string to dict or list). LLM may output something like this $\langle$\{``tofu'': ...\{``physical'': ``color'': ``white\}\}$\rangle$. There is a missing quotation marks of word white. The whole content cannot be parsed in JSON format. Therefore, we need examples of knowledge in JSON format to guide LLM. The token used will also be less.

% ==========

% For example,Fig~\ref{fig:graph_gen_pipeline}) or 
% ``tofu'':
% \{
% ``physical'': \{``texture'': ``soft and smooth'', ``shape'': ``block or curd-like'', ... \},
% ``composition'': \{``main ingredient'': ``soybeans'', ``coagulant'': ``calcium sulfate or magnesium chloride'' \},
% ... \}

% Andong: example of GKG generation, object usage

% INPUT:

% \#System\#: You are a knowledgeable assistant. You know a lot about object usages.

% \#User\#: Please tell me 5 usages of water. The answer should be short and precise following the format '\textless{}the thing applied on\textgreater{}: \textless{}how to apply\textgreater{}'. The answer is a list in simple JSON format where each item is a dict and the key is \textless{}the thing applied on\textgreater{}.

% \#Assistant\#: [\{"human": "hydration"\}, \{"dirt": "cleaning"\}, \{"food": "cooking"\}, \{"crop": "irrigation"\}, \{"electricity": "power generation"\}].

% \#User\#: Please tell me 5 usages of salt. The answer should be short and precise following the format '\textless{}the thing applied on\textgreater{}: \textless{}how to apply\textgreater{}'. The answer is a list in simple JSON format where each item is a dict and the key is \textless{}the thing applied on\textgreater{}.

% \#Assistant\#: [\{"food": "preserving"\}, \{"stained coffee mugs": "cleaning"\}, \{"clothes": "removing stains from"\}, \{"grease fires": "extinguishing"\}, \{"cutting boards": "refreshing"\}],

% \#User\#: Please tell me 5 usages for cornstarch. The answer should be short and precise following the format '\textless{}the thing applied on\textgreater{}: \textless{}how to apply\textgreater{}'. The answer is a list in simple JSON format where each item is a dict and the key is \textless{}the thing applied on\textgreater{}.

% OUTPUT:

% \#Assistant\#: [\{"sauce": "thickening"\}, \{"batter": "making crispy"\}, \{"body powder": "absorbing moisture"\}, \{"starch": "making"\}, \{"playdough": "creating homemade"\}]


\subsection{Situated Commonsense Knowledge Graph (SCKG)}
\label{sec:method_situated_commonsense_knowledge_graph}
% \input{algorithms/alg3}

% We generate Situated Knowledge Graph $\mbox{\boldmath$G$}_{sk}$ by combining Video Content Graph $\mbox{\boldmath$G$}_{v}$ and General Knowledge Graph $\mbox{\boldmath$G$}_{gk}$ as demonstrated in Algorithm~\ref{algo:situated_commonsense_knowledge_graph_generation}. For each object $o_{i}$ and each action $a_{t}$, we instruct LLM to analyze their functions and their logical relationships with others to generate situated knowledge. The prompt template is: $\langle$\textit{video content} $g_{v}$, \textit{general knowledge} $k_{g}$, \textit{situated knowledge examples} $\pi$, \textit{generation goal} $\omega$, \textit{output format} $\phi$$\rangle$. The \textit{video content} is a textualized version of $\mbox{\boldmath$G$}_{v}$ and \textit{general knowledge} corresponds to the select object $o_{i}$ or action $a_{t}$. Similar to the \textit{general knowledge examples} for $\mbox{\boldmath$G$}_{gk}$, \textit{situated knowledge examples} relate to a \textit{situated knowledge aspect} (\eg, \textit{counterfactual} and \textit{purpose}). However, as shown in Algorithm~\ref{algo:situated_commonsense_knowledge_graph_generation}, we do not provide the examples manually in advance but propose our \textbf{Self-Few-Shot Prompting} technique by utilizing former generated situated knowledge as examples.

% We link the knowledge descriptions to generate situated knowledge graphs via causal or relevant relations.

% \subsubsection{Situated Knowledge Generation via Few-Shot Self-Prompting}
% \noindent\textbf{Self-Few-Shot Prompting for Concrete and Specific Knowledge Generation.} The need for this technique is that we find, without examples, the LLM may generate situated knowledge that is semantically correct but less concrete and specific. For instance, without examples, if we ask LLM with \textit{generation goal}: ``What would happen if the person did not use ground pork during cooking mapo tofu?'' with \textit{output format}: ``The answer should be short, precise, and specific'', the model may still answer ``The dish would lack flavor and texture'', which is correct but too general and not ``situated'' enough. However, we cannot manually provide examples in advance to instruct LLM how ``specific'' the generated knowledge should be as the knowledge is situated on video $v$. To tackle the problem, as shown in Algorithm~\ref{algo:situated_commonsense_knowledge_graph_generation}, we use the generated situated knowledge of other objects or actions as examples. We repeat the whole process in multiple iterations and update the knowledge in the examples. For instance, the consequence of not using ground pork answered by LLM would finally be ``The dish would lack meaty flavor, texture, and richness.''

% Here, we do not provide the examples manually beforehand, so the approach improves the efficiency of the method and allows for a more streamlined generation of the Situated Knowledge Graph.
% The motivation is that we find, without examples, that the LLM may generate situated knowledge that is semantically correct but less concrete and specific. For instance, without examples, if we query the LLM with a \textit{generation goal} such as, "What would happen if the person did not use ground pork during cooking mapo tofu?" and an \textit{output format} stating, "The answer should be short, precise, and specific," the model may still respond with "The dish would lack flavor and texture." While this answer is correct, it is too general and insufficiently "situated."
% However, it is not feasible to manually provide examples in advance to instruct the LLM on the desired level of specificity, as the knowledge is situated on video $v$. 
% \bo{check if duplicate with the above description:}

% % as illustrated in Algorithm~\ref{algo:situated_commonsense_knowledge_graph_generation}, 
% To address this challenge, we utilize the generated situated knowledge of other objects or actions as examples. We repeat the entire process in multiple iterations, updating the knowledge in the examples accordingly. For example, the consequence of not using ground pork, as answered by the LLM, would ultimately be, "The dish would lack meaty flavor, texture, and richness, resulting in a vegetarian version of mapo tofu."

% The prompt template is defined as: $\langle$\textit{video content} $g_{v}$, \textit{general knowledge} $k_{g}$, \textit{situated knowledge examples} $\pi$, \textit{generation goal} $\omega$, \textit{output format} $\phi$$\rangle$. The \textit{video content} is a textual representation of $\mathbf{G}_{v}$, and the \textit{general knowledge} corresponds to the selected object $o_{i}$ or action $a_{t}$. Similar to the \textit{general knowledge examples} for $\mathbf{G}_{gk}$, the \textit{situated knowledge examples} are associated with a \textit{situated knowledge aspect} (\eg, \textit{counterfactual} and \textit{purpose}).

% Commonsense knowledge differs from encyclopedic knowledge in that it deals with general knowledge rather than the details of specific entities~\cite{tandon2018}.
In our work, Situated Commonsense Knowledge Graph $\mbox{\boldmath$G$}_{sk}$ is a generated novel knowledge graph conditioned on the forementioned SKG and GKG of the same dynamic situation. 
% For each node (object $o_{i}$ or action $a_{t}$), we apply the relevant general knowledge from GKG to analyze their roles and logical relationships within the given situation represented by SKG.
Here, we illustrate the importance and complexity of generating situated commonsense knowledge through a simple example. Let's consider a counterfactual scenario where we want to ask about the effects of not using cornstarch in the preparation of mapo tofu (as demonstrated in Figure~\ref{fig:graph_gen_pipeline}). Relying solely on general knowledge of cornstarch (\eg, it is a powdery substance) would not provide us with the correct answer. Instead, we need to leverage the situated information of cornstarch from SKG (\eg, ``The person mixes cornstarch with water and adds the mixture to the soup.'') and integrate it with relevant general knowledge from GKG (\eg, ``Cornstarch can be used as a thickening agent.'') to deduce the effects. The result for the example would be ``The sauce would lack thickness and the dish would have a thinner consistency.''.

Intuitively, the prompt of situated commonsense knowledge generation could be a quadruple: $\langle$\textit{video content} $g_{v}$, \textit{general knowledge} $k_{g}$, \textit{generation goal} $\omega$, \textit{output format} $\phi$$\rangle$. However, our experiments discover that LLM may generate situated commonsense knowledge that is semantically correct but lacks concrete and specific representations. For instance, although we query the LLM with a \textit{generation goal} and an \textit{output format} stating (such as, ``What would happen if the person did not use ground pork during cooking mapo tofu?'' and ``The answer should be short, precise, and specific''), the model may still respond with ``The dish would lack flavor and texture.'' While this answer is correct, it is too general and irrelevant to situated conditions.
Meanwhile, it is not feasible to manually provide examples in advance to instruct the LLM on the desired level of specificity, as the knowledge is situated on video $v$. 
Therefore, we propose a method called Few-Shot Self-Prompting to tackle the problem.

\textbf{Few-Shot Self-Prompting.} Few-shot self-prompting leverages previously generated situated commonsense knowledge as examples. In this approach, the prompt comprises a pentad: $\langle$\textit{video content} $g_{v}$, \textit{general knowledge} $k_{g}$, \textit{situated commonsense knowledge examples} $\pi$, \textit{generation goal} $\omega$, \textit{output format} $\phi$$\rangle$. Please see the details of the Algorithm in Supplementary Materials.

As illustrated in Figure~\ref{fig:graph_gen_pipeline}, the \textit{situated knowledge examples} $\pi$ are constructed using previously generated knowledge concerning the consequences of not using a specific ingredient (in this case, only ``cornstarch'' is shown due to content limitations in Figure~\ref{fig:graph_gen_pipeline}). The newly generated knowledge is then added to the \textit{situated commonsense knowledge examples}. Over time, this process results in increasingly concrete and specific situated commonsense knowledge. We demonstrate the final generation results: the consequence if not using ground pork would be ``The dish would lack meaty flavor, texture, and richness, resulting in a vegetarian version of mapo tofu.'' The intuition of the proposed Few-Shot Self-Prompting technique might be that the knowledge of other objects or actions can serve as a contrast to the current one. Leveraging the model's in-context learning ability can generate more concrete and specific knowledge about the target object or action.

Using our Few-Shot Self-Prompting technique, we employ a selection of situated commonsense knowledge perspectives. These include the ability to consider \textit{counterfactual} scenarios for an object or action, understand the \textit{purpose of an action} within a given situation, and recognize the \textit{contribution of an object} to the process.
% represented as $\{\eta_{i}^{obj}\}$, $\{\eta_{i}^{act}\}$ in Algorithm~\ref{algo:situated_commonsense_knowledge_graph_generation}
Notably, our experimental findings indicate that even just two iterations of knowledge generation yield high-quality knowledge outcomes. Ultimately, this process culminates in the acquisition of SCKG $\mbox{\boldmath$G$}_{sk}$.


% ==========

% highlight points:

% why we need each prompt component

% 1. The naive way, only having ``Video content'' (to make the knowledge situated) and ``Generation goal''. We may get wordy and non-specific knowledge.

% 2. The reason of having ``Output format'' is similar to GKG

% 3. However, with ``Video content'' + ``Generation goal'' + ``Output format'', the generated knowledge is not specific and concrete enough. Therefore, we add self few shot prompting (``SK examples'') is shown in Sec 3.3

% 4. However, still, the generated knowledge can be situated but may miss some points. We provide ``General knowledge'' explicitly in prompt design to guide the LLM. For example, without ``General knowledge'', asking LLM ``Why using cornstarch'', the model could answer ``Thickening the soup''. With ``General knowledge'' which shows the usges of cornstarch include ``thickening agent'' and ``coating and frying'', now model will answer ``Thickening the soup and coating tofu''.

% ==========


% ==========
% Andong; example of SKG generation, object, counterfactual

% \#System\#: You are a helpful, pattern-following assistant. You are very good at deciphering a video, such as summarizing video content, figuring out related commonsense knowledge, and identifying the inner logic. As a commonsense-driven assistant, your task is to analyze a video (length: 119 seconds) that showcases a person introducing 6 cooking steps of mapo tofu.

% The steps are described in a specific format of '[Step N (from <timestamp> to <timestamp>): detailed description of cooking actions]' as follows: [Step 1 (from <16 sec> to <30 sec>): cut tofu into square pieces] ...

% Objects appeared in different frames are described in a specific format of '[Objects at <timestamp>: object(s): attributes of objects]' or '[Objects from <timestamp> to <timestamp>: object(s): attributes of objects]' as follows: [Objects at <0 sec>: tofu: small, square, creamy tofu.] ...

% The relationship of objects are in different frames in format of ‘[object 1 and object 2 at <timestamp>: relationship]’: [tofu and knife at <21 sec>: knife cuts tofu into small squares.] ... 

% The background knowledge of objects appeared in the video is:
% 'cornstarch':{ 'physical': {'state': 'powder', 'color': 'white', ...

% BEFORE:

% \#User\#: What would happen if the person did not use ground pork during cooking mapo tofu? The answer should be direct, precise, short, and within 20 words in one sentence without any comma. Word 'ground pork' should not be included in the answer.

% \#Assistant\#: The dish would lack flavor and texture.

% AFTER

% \#User\#: What would happen if the person did not use water during cooking mapo tofu? The answer should be direct, precise and short and within 20 words in one sentence without any comma. Word 'water' should not be included in the answer.

% \#Assistant\#: The dish would lack moisture, resulting in a dry and less saucy version of mapo tofu.

% \#User\#: What would happen if the person did not use mapo tofu paste during cooking mapo tofu? The answer should be direct, precise and short and within 20 words in one sentence without any comma. Word 'mapo tofu paste' should not be included in the answer.

% \#Assistant\#: The dish would lose its signature flavor and spiciness, resulting in a dish that is not mapo tofu.

% \#User\#: What would happen if the person did not use ground pork during cooking mapo tofu? The answer should be direct, precise and short and within 20 words in one sentence without any comma. Word 'ground pork' should not be included in the answer.

% \#Assistant\#: The dish would lack meaty flavor, texture, and richness, resulting in a vegetarian version of mapo tofu.

% ==========

\subsection{Question and Answer Generation}
\label{sec:method_qa_gen}

Utilizing above three graphs, we generate question-answer pairs to assess the model's capability to make accurate inferences. This evaluation process leverages both factual information specific to a given situation and the essential commonsense knowledge required. To accomplish this, we can adopt two approaches: \textbf{(1)} Manual question-answer templates in a bottom-up manner, where we design question templates and provide corresponding answers based on the graphs. \textbf{(2)} Automatic question generation by utilizing a LLM in a top-down manner.

% Based on the above three graphs, Situated Knowledge Graph (SKG), General Knowledge Graph (GKG), and Situated Commonsense Knowledge Graph (SCKG), we generate question-answer pairs to evaluate the model’s ability to make appropriate inferences by taking advantage of both factual information within a given scenario and the necessary commonsense knowledge. We can achieve this by either manual question-answer templates in a bottom-up manner or automatic question generation by leveraging an LLM in a top-down manner.

\begin{table}[h]
    % \setlength{\abovecaptionskip}{0pt}
    % \setlength{\belowcaptionskip}{0pt}
    \caption{Question template types for Bottom-up QA generation}
    %\tiny %\scriptsize
    \footnotesize
    \centering
    \begin{threeparttable}
    \begin{tabular}{ll}
    \toprule
    % \multicolumn{2}{l}{Reasoning   types} \\
    % \cmidrule(lr){1-2}
    \textbf{Object counterfactual} & vanilla (obj) \\
    (\eg, What would happen if & + obj attributes \\
    the person did not use…) & + obj-obj relationships \\
     & + obj attribute + obj-obj relationship \\
     & + obj general knowledge \\
    \cmidrule(lr){1-2}
    \textbf{Object contribution} & vanilla (obj) \\
    (\eg, Why the person & + obj attributes \\
    use...) & + obj-obj relationships \\
     & + obj attribute + obj-obj relationship \\
     & + obj general knowledge \\
    \cmidrule(lr){1-2}
    \multicolumn{2}{l}{\textbf{Object reasoning}} \\
    \multicolumn{2}{l}{(\eg, What are the two objects which \textless{}interaction\textgreater{})} \\
    \cmidrule(lr){1-2}
    \textbf{Action counterfactual} & vanilla (act) \\
    (\eg, What would happen if & + before / after action \\
    the person did not…) & + before / after action + obj attr / rela \\
    \cmidrule(lr){1-2}
    \textbf{Action purpose} & vanilla (act) \\
    (\eg, Why the person...) & + before/after action \\
     & + before / after action + obj attr / rela \\
    \cmidrule(lr){1-2}
    \multicolumn{2}{l}{\textbf{Action possibility}} \\
    \multicolumn{2}{l}{(\eg, What mistake might the person make if \textless{}possibility\textgreater{})} \\ %\rowcolor{gray!20} 
    \bottomrule
    \end{tabular}
    % \begin{tablenotes}
    % \footnotesize
    % \item 
    % \end{tablenotes}
    \end{threeparttable}
    \label{tab:method_ques_templates}
\end{table}

\subsubsection{Bottom-up QA Generation}
\label{sec:method_rule_based_qa_gen}

We manually design question templates in multi hog way combing both ``situation'' and ``commonsense'' (see the template types in Table~\ref{tab:method_ques_templates}). For one object / action, we find the connected edges in the three graphs. Next, we design question templates that jump from edges in Situated Knowledge Graph or General Knowledge Graph to those in Situated Commonsense Knowledge Graph. Concretely, for example, the template of question type ``obj counterfactual + obj attribute + obj-obj relation'' as illustrated in Table~\ref{tab:method_ques_templates} would be ``What would happen if the person did not use the \textit{\textless{}obj attribute\textgreater{}} and \textit{\textless{}obj-obj relation\textgreater{}}?''(see one concrete question example concerning ``cornstarch'' in Figure~\ref{fig:teaser}). The model needs to first do spatiotemporal reasoning to identify the object by  \textit{\textless{}obj attribute\textgreater{}} and \textit{\textless{}obj-obj relation\textgreater{}} (\eg, ``white substance'' and ``dissolved in water in glass''). Next, the model needs to do situated commonsense reasoning to understand the consequence if that object was not used. In such way, we can comprehensively assess model's situated commonsense reasoning ability. Note that we also present some easier templates (\eg, ``vanilla obj counterfactual'') which are single hog.

% We design question templates to reflect the diverse task types and the specific question key points.
% According to the edges from VG and GKG with those from SKG, the template is able to compose both elementary components within the situations and reasoning logics for questions. 
% For instance, for question type ``object counterfactual + obj attribute + obj-obj relationship'' as illustrated in Table~\ref{tab:method_ques_templates}, we select edges that signify \textit{object attributes} and \textit{object-object relationships} from VG. Subsequently, for the same \textit{object}, we choose edges that represent the \textit{counterfactual} situations about an \textit{object} from SKG. By merging these edges and utilizing the corresponding question template (for the question type, the template can be ``What would happen if the person did not use the \textit{\textless{}obj attribute\textgreater{}} object \textit{\textless{}obj-obj relationship\textgreater{}}?''), we can generate questions as demonstrated in Figure~\ref{fig:question_examples}. These templates enable the generated questions to assess the model's spatiotemporal and commonsense reasoning capabilities within a given context.

\subsubsection{Top-down QA Generation}
\label{sec:method_top_down_qa_gen}

Bottom-up QA generation offers control over question quality and difficulty but lacks flexibility in creating diverse question types. To overcome this limitation, we suggest a top-down approach for QA generation. We design a structured prompt $\langle$\textit{video content}, \textit{integrated graph}, \textit{QA examples}, \textit{generation goal}, \textit{output format}$\rangle$. The \textit{integrated graph} combines SKG, GKG, and SCKG. \textit{QA examples} are randomly selected from bottom-up generated QAs, while the \textit{generation goal} instructs the LLM to create multi-hop questions based on multiple edges from \textit{integrated graph}. This prompt design maintains a strong connection between the generated QAs and graphs, significantly reducing the likelihood of model hallucination when compared to basing QAs solely on video content.

However, the top-down approach has its drawbacks—it is resource-intensive and slow. With the three graphs involved, top-down QA generation takes a few seconds to generate one question, whereas the bottom-up method generates the entire benchmark in the same time. In this paper, we primarily use the bottom-up method for creating the benchmark, but we discuss top-down generation case studies in the Supplementary Material.

% \subsubsection{question-answer and graphs}
% \label{sec:method_qa_graph_alignment}

% ==========

% example of rationale

% Q: What would happen if the person did not use the white substance dissolved in water in glass?

% Choices:

% A. The dish would be completely different.

% B. The dish would lack thickening agent. (correct)

% C. The dish would lack seasoning and taste bland.

% D. The dish would lose its signature flavor.

% Reasoning process generated by LLM

% 1. From [object attributes], we can see that cornstarch is white.

% 2. From [object-object relations], we can see that cornstarch is dissolved in water in glass.

% 3. In the video, Step 2 (from 32 sec to 40 sec): put cornstarch in a small bowl and mix with water

% 4. Step 6 (from 98 sec to 105 sec): add cornstarch and stir gently

% 5. From [General Knowledge Graph], we know that cornstarch can be used as thickening agent to thicken soups.

% 6. From the video, from 32 sec to 40 sec, we can see that cornstarch is put in a small bowl and mixed with water to form a paste.

% 7. This paste is then added to the dish (from 98 sec to 105 sec) to thicken the sauce.

% 8. Therefore, the correct answer is The dish would lack thickening agent.

% 9. The other choices can be eliminated because they are not the correct consequences if the person did not use cornstarch.


\subsection{Quality Valiation}
We invite human helpers to assess the quality by inspecting a subset of the graphs and QAs. We find 94\% of QA pairs are valid. Please see Supplementary Materials for details.

% You must include your signed IEEE copyright release form when you submit your finished paper.
% We MUST have this form before your paper can be published in the proceedings.

% Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
% \url{https://www.computer.org/about/contact}.

% ==========
\subsubsection{Data Source}
We created the benchmark based on videos of the two public video datasets about daily activities, as detailed in Table~\ref{tab:dataset_sources_youcook2_homage}.
% They have high-quality videos and captions, and the videos exhibit entities and logical relationships between actions. 
% YouCook2~\cite{zhou2018towards} and HOMAGE~\cite{rai2021home}

\begin{table}[t]
    \setlength{\abovecaptionskip}{0pt}
    \setlength{\belowcaptionskip}{0pt}
    \caption{Video Data Source}
    %\tiny %\scriptsize
    \scriptsize
    \centering
    \begin{threeparttable}
    \begin{tabular}{p{1.2cm}C{1cm}C{0.5cm}C{0.5cm}C{0.1cm}C{0.1cm}C{0.6cm}C{0.6cm}}
    \toprule
    Data Source & \multicolumn{3}{c}{Content} & \multicolumn{4}{c}{Annotation} \\
     & Obj & Act & Scene & Obj & Act & Temporal & Relations \\
    \cmidrule(lr){2-4}\cmidrule(lr){5-8}
    HOMAGE~\cite{rai2021home} & daily & daily & home & \checkmark & \checkmark & \checkmark & \checkmark \\
    YouCook2~\cite{zhou2018towards} & ingredients & cooking & kitchen & \checkmark & \checkmark & \checkmark &  \\
    \bottomrule
    \end{tabular}
    % \begin{tablenotes}
    % \footnotesize
    % \item 
    % \end{tablenotes}
    \end{threeparttable}
    \label{tab:dataset_sources_youcook2_homage}
\end{table}


\noindent\textbf{YouCook2}~\cite{zhou2018towards} is a comprehensive collection of instructional cooking videos from YouTube. It features over 2,000 videos, spanning 89 different recipe categories, where each video is annotated with detailed step-by-step instructions.

\noindent\textbf{HOMAGE}~\cite{rai2021home} consists of 1,752 video clips including 75 human daily activities within home environments. The dataset is richly annotated with action labels, object information, and spatial-temporal relationships.


==> tables/related.tex <==
\begin{table*}[t]
    \resizebox{1\linewidth}{!}
    {
    \small
    \setlength{\tabcolsep}{2pt}
	\begin{tabular}{lccccccc}
	\toprule
         \multirow{2}{*}{Dataset}  & Question &  \multirow{2}{*}{Rationales}   & Diverse & {Goal-driven}   & Interaction & {Counterfactual} &  \\
         & Answering  &  & Scenarios & Questions & of soft objects & Property Dynamics  \\
         CRAFT~\citep{ates2020craft} & $\surd$ &  $\surd$ &  $\times$ & $\times$ & $\times$ & $\times$  \\
         CLEVRER~\citep{yi2019clevrer} & $\surd$ &  $\surd$ &  $\times$ & $\times$ & $\times$ & $\times$    \\
         Physion~\citep{bear1physion} & $\times$ &  $\times$ &  $\surd$ & $\times$ & $\surd$ & $\times$   \\
         ComPhy~\cite{chen2022comphy} & $\surd$ &  $\surd$ &  $\times$ & $\times$ & $\surd$ & $\surd$    \\ 
         CRIPP-VQA~\cite{patel2022cripp}  & $\surd$ &  $\surd$ &  $\times$ & $\surd$ & $\times$ & $\times$  \\
        \midrule 
        \dataset (Ours) & $\surd$ &  $\surd$ &  $\surd$ & $\surd$ & $\surd$ & $\surd$  \\
        \bottomrule 
	\end{tabular}
	}
	\caption{Comparison between \dataset and other visual question benchmarks.}
	\label{tab:dataset_comparison}
\end{table*}
